A Rademacher Complexity Based Method fo rControlling Power and Confidence Level in Adaptive Statistical Analysis

While standard statistical inference techniques and machine learning generalization bounds assume that tests are run on data selected independently of the hypotheses, practical data analysis and machine learning are usually iterative and adaptive processes where the same holdout data is often used for testing a sequence of hypotheses (or models), which may each depend on the outcome of the previous tests on the same data. In this work, we present RadaBound a rigorous, efficient and practical procedure for controlling the generalization error when using a holdout sample for multiple adaptive testing. Our solution is based on a new application of the Rademacher Complexity generalization bounds, adapted to dependent tests. We demonstrate the statistical power and practicality of our method through extensive simulations and comparisons to alternative approaches.

==> 01_introduction_old.tex <==
\section{Introduction}
The goal of data analysis and statistical learning is to model a stochastic process, or distribution, that explain an observed data. A major risk in statistical learning is \emph{overfitting}, that is, learning a model that fits well with the observed data but does not predict new data. The standard practice in machine learning is to split the data into \emph{training} and \emph{holdout} (or testing) sets. A learning algorithm then learns a model using the training data and tests the model on the holdout set to obtain a confidence interval for the expected error or for the value of the loss function of the model. If the process halts after a single iteration, then the statistical analysis is easy. However, in most cases, the learning process is iterative and adaptive. One uses successive tests for model selection, feature selection, parameter tuning, etc., and the choice of the tests themselves often depends on the outcomes of previous tests. 

Ideally, each hypothesis should be tested on a fresh data sample. However, it is common practice to reuse the same holdout data to evaluate a sequence of hypotheses. While widespread, this practice is known to lead to \emph{overfitting}; that is, the learned model becomes representative of the sample rather than the actual process. Evaluating the accumulated error in testing a sequence of related hypothesis on the same data set is a major challenge in both machine learning and modern statistics. In machine learning, the problem of ``\emph{preventing overfit}'', is usually phrased and analyzed in terms of bounding the generalization error~\cite{ShalevSBD14}. In inference statistics, the goal is controlling the Family Wise Error Rate (FWER), or the False Discovery Rate (FDR) of a sequence of hypothesis tests~\cite{benjamini1995controlling}.

\paragraph{Our Results:}
We develop and analyze \algo{}, a rigorous, efficient, and practical procedure for online evaluation of the accumulated generalization error in a sequence of statistical inferences applied to the same sample. \algo{}  can evaluate fully adaptive sequences of tests. The choice of a test may depend on the information obtained from previous tests, and the total number of tests is not fixed in advance. 

One way to quantify the risk of overfitting after $k$ queries is by considering the probability of the condition defined by the results of the first $k$ queries. If the probability of such condition is close to 1, the results of the queries evaluated so far do not significantly restrict the sample space, and there is, therefore, no risk of overfitting. Viceversa, if the probability of the observed condition is small, the sample space defined by the true distribution conditioned on the results of the queries is noticeably different from the true distribution, and there is thus a significant risk of overfitting. In general, it is hard to bound the probability of the observed condition as the true distribution over the samples is unknown. However, in the special case for which the queries being considered correspond to evaluating the average of functions (such as evaluating the average risk or loss functions of alternative learning procedures), we can design an adaptive process based on an empirical estimate of the Rademacher Complexity of the set of queries which correctly bounds this probability and correspondingly halts the procedure when the risk of overfitting exceeds a certain threshold fixed by the user.

Our method builds on the concept of Rademacher Complexity~\cite{BartlettBL02,Koltchinskii01} that has emerged as a
powerful alternative to VC-dimension and related  uniform convergence methods for
characterizing generalization error and sample complexity. A fundamental advantage of the Rademacher Complexity approach in contrast to standard uniform convergence tools, such as
 VC-dimension, that capture the complexity with respect the worst case input
 distribution, is that it yields a data-dependent bound as it
is computed with respect to the input (sample) distribution, and can be efficiently approximated from the sample. 

Our solution employs three major components: (1) For a set of functions chosen independent of the sample, the \Rade{}~\cite{BartlettBL02,Koltchinskii01} provides a powerful and efficient bound on the error in estimating the expectations of all these function using one sample; (2) As long as the outcome of the sequence of tests does not significantly overfit to the sample, conditioning on these outcomes has only a minor effect on the distribution; and (3) The \Rade{} of a sequence of tests can be estimated efficiently form a given sample, requiring similar computation time as running the actual tests. 

To fully utilize our technique, we need computationally efficient methods for rigorously estimating the Rademacher Complexity from a sample. We introduce two novel methods based on Bernstein's inequality for martingales~\cite{freedman1975tail} and the Martingale Central Limit Theorem~\cite{hall2014martingale}. 
Our analysis and extensive experiments prove and demonstrate that  our method guarantees statistical validity while retaining statistical power and practical efficiency.
\paragraph{Related Work:}
Classic statistics offers a variety of procedures for controlling the Family Wise Error Rate (FWER), ranging from the simple Bonferroni~\cite{bonferroni1936teoria} to Holm's step-down~\cite{holm1979simple} and Hochberg's step-up procedures~\cite{hochberg1988sharper} in the context of multiple hypotheses testing. While controlling the FWER under weak assumptions about the hypotheses, these methods are too conservative, giving many false negative results, in particular for large sets of hypotheses. Less conservative procedures, such as Benjamini and Hochberg~\cite{benjamini1995controlling}, which control the False Discovery Rate (FDR) (i.e., the expected fraction of false discoveries), still do not scale up well for a very large number of hypotheses. However, all these procedures cannot be applied in the adaptive setting, as they require for the set of hypotheses to be fixed at the beginning of the testing procedure (i.e., before any data evaluation).

A series of recent papers~\cite{Dwork15generalization,dwork2015reusable,dwork2015preserving} explored an interesting relation between ``\emph{Differential Privacy}''~\cite{dwork2006calibrating} and overfit prevention in adaptive analysis. The basic idea is to limit the user access to the holdout data so that the answers to the sequence of queries is differentially private. A differentially private access to the holdout data limits the risk of overfitting to that data set. Unfortunately, the practical application of this elegant mathematics is limited. Differential privacy is achieved through random perturbation of the data (or the reply to the queries). The higher the number of adaptive queries, the larger the required perturbation. However, the amount of perturbation is limited by the need to preserve the actual signal in the data. As a result, rigorous application of this approach is either limited to a small number of queries or is computationally intractable~\cite{dwork2015preserving}, making it less useful than alternative methods~\cite{hardt2014preventing,steinke2015interactive}. 
Our experiments in Section 5 show that \algo{} allows orders of magnitude reduction of the required holdout dataset compared to Dwork et al.'s method~\cite{Dwork15generalization} while offering the same guarantees. Further, our technique is much simpler as it does not require any introduction of additional noise.
We discuss in detail the advantages of our solution compared to ~\cite{Dwork15generalization} in Section~\ref{sec:dwork}.
% proved lower bound (under standard cryptographic assumptions) showing that no computationally
% efficient algorithm for this method can give non-trivial error on quadratic (in the data size) adaptively chosen functions.
A more practical solution for a restricted setting inspired by machine learning competitions was presented in~\cite{blum2015ladder}. Their solution, ``\emph{the Ladder}'', 
provides a loss estimate only for those that made a significant improvement over the previous best. This restricted setting allows to sidestep the hardness results discussed in~\cite{hardt2014preventing,steinke2015interactive}.
% \section{Preliminaries}
% \paragraph{Rademacher Complexity}
% %Our solution is based on iterative applications of Rademacher Complexity bounds.
% %The Rademacher Complexity measure is obtained through a simple symmetrization argument. 
% Let $\bar{x}=(x_1,\dots,x_m)$ be a sample from a distribution $\cal D$, and let $\cal F$ be a set of functions defined on the support of $\cal D$, chosen independently of the sample $\bar{x}$.
% % Assume that for all $f\in {\mathcal F}$ we estimate the expectation of $f$ in $\cal D$, $\Expe{\cal D}{f}$,by $\frac{1}{m}\sum_{i=1}^m f(x_i)$, its empirical expectation in $\bar{x}$.  I.e., we use one sample of $m$ independent items to estimate the expectations of all functions in $\cal F$. We apply Rademacher Complexity to bound the maximum error of all these estimate. 
% %$$E[\Psi ({\cal F},\bar{x}) = \sup_{f\in{\cal F}} |\frac{1}{m}\sum_{i=1}^m f(x_i)- E_{\cal D}[f]|],$$
% Let $\sigma=(\sigma_1,\dots,\sigma_m)$ be a vector of $m$ independent Rademacher variables, such that for each
% $i$, $\Prob{\sigma_i=1}=\Prob{\sigma_i=-1}=1/2$. 

% \begin{definition}{\cite{ShalevSBD14}}\quad
% \begin{enumerate} 
% \item The {\em Empirical Rademacher Complexity} of $\cal
% F$ with respect to a sample $\bar{x}=\{x_1,\dots,x_m\}$ is:\\
% $$R^{\cal F}_{\bar{x}} =E_\sigma \left [\sup_{f\in {\cal
%       F}}\frac{1}{m} \sum_{i=1}^m |f (x_i)\sigma_i |\right].$$
%  \item The {\em Rademacher Complexity} of $\cal
% F$ for samples of size $m$ is defined as:
% %the expectation of the empirical Rademacher Complexity over all samples of size $m$,
%             $$R^{\cal F}_m=\Expe{\bar{x}\sim{\cal D}^m}{R^{\cal F}_{\bar{x}}}.$$
%             \end{enumerate}
%     \end{definition}
% %Taking the expectation over the distribution of training sets, we define
% %the Rademacher Complexity of the set $\cal F$ with respect to the
% %distribution $\cal D$ as
% %  $$R_{m,{\cal F}}=E_{\bar{z}\sim {\cal D}}\left [R_{{\cal F},\bar{z}}\right ].$$
% The fundamental relation between the \Rade of a given class of functions $\mathcal{F}$ and the generalization error in estimating the expectations of all function in $\cal F$  is given in the following theorem~\footnote{In our setting, in order apply the result with absolute value we implicitly assume that for any $f\in{\cal F}$ we also have $-f\in {\cal F}$, that is, we assume that $\cal F$ is \emph{closed under negation}.}
% \begin{theorem}{~\cite{ShalevSBD14}, Lemma 26.2}
% \label{th:Ra}
% %$$\E_{S} \left [\sup_{f\in {\cal F}} \left ( \E_{\cal D} [f(z)]- \frac{1}{m} \sum_{i=1}^m f(z_i) \right ) \right] \leq 2 R_{m, {\cal F}}.$$
% $$\Expe{\bar{x}}{\Psi ({\cal F}_k,\bar{x})}=\Exp{\sup_{f\in{\cal F}} |\frac{1}{m}\sum_{i=1}^m f(x_i)- E_{\cal D}[f]|}
% %\E_{\bar{x}} \left [\sup_{f\in {\cal F}} \left ( \E_{\cal D} [f]- \frac{1}{m} \sum_{i=1}^m f(x_i) \right ) \right] 
% \leq 2 R^{\cal F}_m.$$
% \end{theorem}

% For algorithmic applications, two important consequences of this result are that: (a) for bounded functions the generalization error is concentrated around their expectation, and (b) the \Rade 
% can be efficiently estimated from the sample, thus making the bound actually usable in practice. 
% Let us for instance consider the estimation of the \Rade given by $\sup_{f\in {\cal F}_k} \sum_{i=1}^m \sigma_i f(x_i)$, which can be computed using just one vector of Rademacher random variables $\bar{\sigma}=(\sigma_1,\dots,\sigma_m)$. As shown in~\cite{Barlett02}:
% $$\Pr(|R^{\cal F}_m-\sup_{f\in {\cal F}_k} \sum_{i=1}^m \sigma_i f(x_i) |\geq \epsilon)\leq e^{-m\epsilon^2/8},$$
% This, and other similar bounds presented in the literature are obtained by applying  McDiarmid's Inequality~\cite{ShalevSBD14}[Lemma 26.4]. While by using more complex estimation that use multiple vectors of Rademacher random variable and by considering specific properties of the class of functions being considered\footnote{We discuss an estimation that uses McDiarmid's inequality based on the novel use of multiple vectors of Rademacher Random Variables in Appendix~\ref{app:refinedmcdia}.}, for practical applications, we obtain significantly better bounds by applying the Martingale Central Limit Theorem.
% \paragraph{Martingales}
% We introduce here some basic concepts relative to martingales which we will use in our derivations
% \begin{definition}{\cite{mitzenmacher2017probability}}
% A sequence of random variables $S_0,S_1,\ldots$ is a martingale with respect to the sequence $X_0,X_1,\ldots$ if, for all $n\geq 0$, the following conditions hold:
% \begin{itemize}
% \item $S_t$ is a function of $X_0,\ldots,X_n$;
% \item $\Exp{|S_t|}\leq \infty$;
% \item $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.
% \end{itemize}
% \end{definition}

% G1iven a sequence of random variables $X_0,X_1,\ldots$, and a random variable $Y$, which generally depends on $X_0,X_1,\ldots$, such that $\Exp{|Y|}\leq \infty$, then 
% \begin{equation*}
% C_i =\Exp{Y|X_i,\ldots,X_0}
% \end{equation*}
% gives a martingale. This general construction is referred as ``\emph{Doob martingale}''~\cite{mitzenmacher2017probability}. 
% Finally, given a martingale sequence $S_0,\ldots,S_t$ we refer to the martingale obtained as:
% \begin{equation*}
% Z_i = S_i - S_{i-1},\quad for\ i=1,\ldots t
% \end{equation*}
% as the ``\emph{Difference martingale}'' (or ``\emph{Martingale Difference Sequence}'') corresponding to $S_0,\ldots,S_t$. Note that, as $S_0,\ldots,S_t$ is a martingale, $\Exp{|Z_t|}\leq \infty$ and for all $i = 1,\ldots,t$ we have $\Exp{Z_i|S_i,\ldots,Z_0} = 0$.

==> 02_radabound_old.tex <==
\section{The \textsc{RadaBound}}
\paragraph{The process:} For concreteness, we focus on the following setup.
We have an holdout sample composed by $m$ independent observations $\bar{x}=(x_1,\dots,x_m)$, each from a distribution $\mathcal{D}$, and parameters $\epsilon,\delta\in (0,1)$ fixed by the user.
In an iterative process, at each step, the user (or an adaptive algorithm) submits a function $f$ and receives an estimate $\ExpeApp{\bar{x}}{f}=\frac{1}{m}\sum_{i=1}^m f(x_i)$  of the ``\emph{ground truth value}'' $\Expe{\mathcal{D}}{f}$.
%confidence interval for $E_{\mathcal{D}} [f]$, the expectation of $f$ in $\mathcal{D}$ ,$$\left [\frac{1}{m}\sum_{i=1}^m f(x_i)-\epsilon, \frac{1}{m}\sum_{i=1}^m f(x_i)+\epsilon \right].$$ 
The user has no \emph{direct access} to the sample $\bar{x}$. That is, he can \emph{only} acquire information regarding $\bar{x}$ from the confidence intervals $\ExpeApp{\bar{x}}{f}\pm\epsilon$ for the expectation $\Expe{\mathcal{D}}{f}$, which the testing procedure has returned as answer to the queries considered so far.
Let $\mathcal{F}_k=\{f_1,\dots, f_k\}$ denote the set of the first $k$ functions evaluated during the adaptive process. The maximum error in estimating the expectations of the $k$ functions is given by: 

\begin{align*}
\Psi \left(\mathcal{F}_k,\bar{x}\right) &= \sup_{f\in\mathcal{ F}_k} |\frac{1}{m}\sum_{i=1}^m f(x_i)- \Expe{\mathcal{ D}}{f}|\\ &= \sup_{f\in\mathcal{ F}_k} |\ExpeApp{\bar{x}}{f}- \Expe{\mathcal{D}}{f}|.
\end{align*}
In this work, we use the expression ``\emph{overfittig}'' as follows: A given set of functions $\mathcal{F}_k$ is said to \emph{overfit the sample} $\bar{x}$ if for any $f\in \mathcal{F}$ the value  $\ExpeApp{\bar{x}}{f}$ evaluated on $\bar{x}$ differs from the \emph{true value} $\Expe{\mathcal{D}}{f}$ by more than the user given threshold $\epsilon$. Our adaptive testing process halts at the first $k$-th step for which for which it cannot guarantee that the probability of overfitting is at most $\delta$, that is, when  $\Prob{\maxErr{\mathcal{F}_k,\bar{x}}\leq \epsilon}\geq 1 -\delta$.

The process is fully adaptive. The choice of the function $f_{k+1}$ evaluated at the $k+1$-th step may depend on the information obtained during the first $k$ steps. We make no assumptions on the processes according to which the functions are adaptively chosen to be tested, nor do we require the total number of tests to be fixed in advance. For simplicity, we assume that all functions are in the range $[0,1]$. More general settings are discussed later in the paper.
\paragraph{Bounding the generalization error for the iterative process:}
The sequence of answers to the queries, $\ExpeApp{\bar{x}}{f_1}\pm\epsilon,\ExpeApp{\bar{x}}{f_2}\pm\epsilon, \dots,\ExpeApp{\bar{x}}{f_k}\pm\epsilon$ defines a filtration 
$\mathcal{L}=\{\mathcal{ D}_k\}_{k\geq 0}$, such that 
$$\mathcal{ D}_0= \mathcal{ D}~~ \mbox{and}~~  \mathcal{ D}_k= \{\mathcal{ D}~|~ \ExpeApp{\bar{x}}{f_1}\pm\epsilon \wedge \dots \wedge \ExpeApp{\bar{x}}{f_k}\pm\epsilon\}.$$ The $k$-th query is chosen with respect to, and is answered in the filtered distribution $\mathcal{D}_{k-1}$.
%Our first step in developing \algo{} is to adapt the Rademacher Complexity results to an iterative, adaptive sequence of queries. 

Let $E_k$ denote the event that the answer to the $k$-th query was within $\epsilon$ of the correct value, that is,  $E_k := |\ExpeApp{\bar{x}}{f}- \Expe{\mathcal{D}}{f_k}|\leq \epsilon$.
%expectations in $\cal D$, 
%$$E_k: \Psi \left(\mathcal{ F}_k,\bar{x}\right) = \sup_{f\in\mathcal{ F}_k} |\frac{1}{m}\sum_{i=1}^m f(x_i)- \Expe{\mathcal {D}}{f}|\leq \epsilon.$$
%\{ \frac{1}{m}\sum_{i=1}^m f_j (x_i)\in [ E_{\mathcal{D}} [f_j]-\epsilon, E_{\cal D} [f_j]+\epsilon] ~|~1\leq j \leq k \}.$$
Then,
$\Prob{\maxErr{\mathcal{ F}_k,\bar{x}}\leq \epsilon}=\Prob{\wedge_{i=1}^k E_k}$, and thus, in the filtration process,
\begin{align}\label{eq:iterativeproc}
\begin{split}
&\Probd{\mathcal{L}}{\Psi (\mathcal{ F}_k,\bar{x})> \epsilon}\\ 
&\qquad\leq \Probd{\mathcal{ D}_0}{\bar{E}_1} + \Probd{\mathcal{ D}_1}{\bar{E}_2} + \ldots 
 + \Probd{{\mathcal{ D}_{k-1}}}{\bar{E}_k}\\ 
& \qquad = \sum_{i=1}^k \frac{\Prob{\bar{E}_i
\wedge (\wedge_{j=1}^{i-1}E_j)}}{\Prob{\wedge_{j=1}^{i-1}E_j}}\\ 
&\qquad\leq \frac{1-\Prob{\wedge_{j=1}^{k}E_j}} {\Prob{\wedge_{j=1}^{k-1}E_j}} \\
& \qquad
= \frac{1- \Prob{\maxErr{\mathcal{ F}_k,\bar{x}}\leq \epsilon}}{\Prob{\Psi (\mathcal{ F}_{k-1},\bar{x})\leq \epsilon}},  
\end{split}
\end{align}
where $\Prob{}{}$ with no subscript refers to probability in the un-filtered distribution $\mathcal{D}$.

The fact that the distribution of the generalization error in the adaptive case, $\Probd{\mathcal{L}}{\maxErr{\mathcal{ F}_k,\bar{x}}> \epsilon}$, is related to the probability of an error in the non-adaptive case, $\Prob{\maxErr{\mathcal{ F}_k,\bar{x}}> \epsilon}$, is not surprising. In order to fit the sample differently than the original distribution $\mathcal{D}$, the process needs to detect a pattern whose frequency is considerably different in the sample compared to the actual distribution $\mathcal{D}$. However, the first query that observes such a pattern is chosen when the process has not yet observed a significant difference between the sample and the distribution. 
This is due to the fact that the process halts as soon as such difference is detected. Thus, the probability of overfitting in $k$ queries is related the to the probability that the sample gives a bad estimate for the correct value of one of the $k$ queries in the non-adaptive case.

The challenge is to compute a tight bound to the probability $\Prob{\maxErr{\mathcal{ F}_k,\bar{x}}\leq \epsilon}$. We achieve this through two novel bounds on estimating the Rademacher Complexity of $\mathcal{ F}_k$.

%We achieve this by relating this value to the Rademacher Complexity of ${\cal F}_k$, and developing two novel tight bounds 
%on estimating the empirical Rademacher Complexity through  \emph{Bernstein's inequality for Martingales}~\cite{freedman1975tail}, and of the \emph{Martingale Central Limit Theorem} (MCLT).
%The process defines a filtration 
%$\{{\cal D}_k= {\cal D}~|~E_k\}_{k\geq 1}$. The main difficulty in the analysis is given by the fact that the known results using Rademacher Averages hold for an independent sample from $\cal D$, while in the adaptive setting we need bounds that hold for the conditional distributions ${\cal D}_k$. 
%Clearly, for every $k$, we have
%\begin{equation*}\label{eq:1}
%\Prob{\Psi ({\cal F}_{k+1},\bar{x})\leq \epsilon ~|~E_k} =\frac{\Probd{\cal D}{E_{k+1}}}{\Probd{\cal D}{E_k}}\end{equation*}
%
%
\section{Bounding $\maxErr{\mathcal{ F}_k,\bar{x}}$ using \Rade{}}
%Our solution is based on iterative applications of Rademacher Complexity bounds.
%The Rademacher Complexity measure is obtained through a simple symmetrization argument. 
%Let $\bar{x}=(x_1,\dots,x_m)$ be a sample from a distribution $\cal D$, and let $\cal F$ be a set of functions defined on the support of $\cal D$, chosen independently of the sample $\bar{x}$.
% Assume that for all $f\in {\mathcal F}$ we estimate the expectation of $f$ in $\cal D$, $\Expe{\cal D}{f}$,by $\frac{1}{m}\sum_{i=1}^m f(x_i)$, its empirical expectation in $\bar{x}$.  I.e., we use one sample of $m$ independent items to estimate the expectations of all functions in $\cal F$. We apply Rademacher Complexity to bound the maximum error of all these estimate. 
%$$E[\Psi ({\cal F},\bar{x}) = \sup_{f\in{\cal F}} |\frac{1}{m}\sum_{i=1}^m f(x_i)- E_{\cal D}[f]|],$$
\begin{definition}{\cite{mitzenmacher2017probability}}  Let $\bar{\sigma}=(\sigma_1,\dots,\sigma_m)$ be a vector of $m$ independent \emph{Rademacher random variables}, such that for all $i$,  $\Prob{\sigma_i=1}=\Prob{\sigma_i=-1}=1/2$. 
The {\em Empirical Rademacher Complexity} of a class of function $\mathcal{
F}$ with respect to a sample $\bar{x}=\{x_1,\dots,x_m\}$, with $\bar{x}\sim \mathcal{D}^m$ is 
\begin{equation*}
R^{\mathcal {F}}_{\bar{x}} = \Expe{\bar{\sigma}}{\sup_{f\in \mathcal{
    F}}\frac{1}{m} \sum_{i=1}^m f (x_i)\sigma_i }
\end{equation*}
The \emph{Rademacher Complexity} of $\mathcal{
F}$ for samples of size $m$ is defined as $R^{\mathcal{F}}_m:=\Expe{\bar{x}\sim\mathcal{ D}^m}{R^{\mathcal{F}}_{\bar{x}}}$.
    \end{definition}
%Taking the expectation over the distribution of training sets, we define
%the Rademacher Complexity of the set $\cal F$ with respect to the
%distribution $\cal D$ as
%  $$R_{m,\mathcal{ F}}=E_{\bar{z}\sim {\cal D}}\left [R_{{\cal F},\bar{z}}\right ].$$

The relation between $\Psi (\mathcal{ F}_k,\bar{x})$ and the Rademacher Complexity of $\mathcal{ F}_k$ is given by the following results~\footnote{In our setting, in order apply the result with absolute value we assume that for any $f\in\mathcal{ F}_k$ we also have $-f\in \mathcal{ F}_k$, i.e., we assume that $\mathcal{F}_k$ is \emph{closed under negation}.}:
%The fundamental relation between the \Rade{} of a given class of functions $\mathcal{F}$ and the generalization error in estimating the expectations of all function in $\cal F$  is given in the following theorems~\footnote{In our setting, in order apply the result with absolute value we implicitly assume that for any $f\in{\cal F}$ we also have $-f\in {\cal F}$, that is, we assume that $\cal F$ is \emph{closed under negation}.}
\begin{lemma}[\emph{Lemma 26.2,} \citealp{ShalevSBD14}] 
\label{th:Ra}
%$$\E_{S} \left [\sup_{f\in {\cal F}} \left ( \E_{\cal D} [f(z)]- \frac{1}{m} \sum_{i=1}^m f(z_i) \right ) \right] \leq 2 R_{m, {\cal F}}.$$
\begin{align*}
\Expe{\bar{x}\sim\mathcal{ D}^m}{\Psi (\mathcal{ F}_k,\bar{x})} &=\Exp{\sup_{f\in\mathcal{ F}_k} |\frac{1}{m}\sum_{i=1}^m f(x_i)- E_\mathcal{ D}[f]|}\\
%\E_{\bar{x}} \left [\sup_{f\in {\cal F}} \left ( \E_{\cal D} [f]- \frac{1}{m} \sum_{i=1}^m f(x_i) \right ) \right] 
&\leq 2 R^{\mathcal{ F}_k}_m.
\end{align*}
\end{lemma}
\begin{lemma}[\emph{Theorem 14.21,} \citealp{mitzenmacher2017probability}]\label{th:Ra2}
Assume that for all $x\in \mathcal{X}$ and $f\in \mathcal{F}_k$ we have $f(x)\in \left[0, 1 \right]$, then:
\begin{equation}\label{Radbound11}
\Prob{\Psi (\mathcal{ F}_k,\bar{x}) > 2R^{\mathcal{F}_k}_m+ \epsilon}\leq e^{-2m\epsilon^2}. 
\end{equation}
\end{lemma}
Note that 
%the bound presented here is stronger than the one in~\cite{mitzenmacher2017probability} as 
in our context (a) we need a one-sided bound, and (b)  for all $x\in \mathcal{X}$ and $f\in \mathcal{F}_k$ we have $f(x)\in \left[0, 1 \right]$.

For algorithmic applications, two important consequences of these result are that: (a) for bounded functions the generalization error is concentrated around their expectation, and (b) the \Rade{} can be estimated from the sample.
In order for this bound to be actually usable in practical applications, it is necessary to compute an estimate of the \Rade{} given the dataset $\bar{x}$, and to bound its error. In the ``\emph{textbook}'' treatment, the difference between Rademacher Complexity and its empirical counterpart is bounded using a second application of \emph{McDiarmid's Inequality}~\cite{Barlett02,ShalevSBD14}. However, this bound is often too loose for practical applications such as ours. 

In this work, we propose an alternative, \emph{direct}, estimate of the \Rade{} and we develop two methods for tightly bounding the estimation error.
% Next we need to bound $R^{\cal F}_m - {R^{\cal F}_{\bar{x}}}$, the error in estimating the Rademacher Complexity of ${\cal F}_{\bar{x}}$ by the empirical Rademacher Complexity using sample $\bar{x}$. The "textbook" treatment of Rademacher Complexity bounds this value by a second application of McDiarmid's Inequality~\cite{Barlett02,ShalevSBD14}. This bound is too loose for application. Instead, we develop two tighter methods for bounding this error.
%For algorithmic applications, two important consequences of these result are that: (a) for bounded functions the generalization error is concentrated around their expectation, and (b) the \Rade{}
%can be efficiently estimated from the sample, thus making the bound actually usable in practice. 
%% consequences of this result are that: (a) for bounded functions the generalization error is concentrated around their expectation, and (b) the \Rade 
%% can be efficiently estimated from the sample, 
%% Let us for instance consider the estimation of the \Rade given by $\sup_{f\in {\cal F}_k} \sum_{i=1}^m \sigma_i f(x_i)$, which can be computed using just one vector of Rademacher random variables $\bar{\sigma}=(\sigma_1,\dots,\sigma_m)$. As shown in~\cite{Barlett02}:
%% $$\Pr(|R^{\cal F}_m-\sup_{f\in {\cal F}_k} \sum_{i=1}^m \sigma_i f(x_i) |\geq \epsilon)\leq e^{-m\epsilon^2/8},$$
%% 
%In the theory literature, the bounds which characterize the relation between generalization error and \Rade{}, and the quality of an estimation of the \Rade{} based on a given sample are proven by applying  McDiarmid's Inequality~\cite{Barlett02,ShalevSBD14} to obtain finite sample bounds. In  Appendix~\ref{app:refinedmcdia} we discuss similar results when using multiple vectors of Rademacher random variables inequality.
%% While by using more complex estimation that use multiple vectors of Rademacher random variable and by considering specific properties of the class of functions being considered\footnote{We discuss an estimation that uses McDiarmid's inequality based on the novel use of multiple vectors of Rademacher Random Variables in Appendix~\ref{app:refinedmcdia}.}, 
%In the next section, we will introduce significantly better finite sample bounds obtained by applying \emph{Bernstein's Inequality for Martingales}, and alternative \emph{asymptotic} bounds using the Martingale Central Limit Theorem. 

==> 03_boundinggenerror.tex <==
\section{Bounding the generalization error using the MCLT}\label{sec:mcltgen}
As in the finite sample bounds, we analyze the estimation process of the Rademacher complexity as a Doob martingale. We will use the following basic definitions:
% \paragraph{Martingales}
% We introduce here some basic concepts relative to martingales which we will use in our derivations.

\begin{definition}{\cite{mitzenmacher2017probability}}
A sequence of random variables $S_0,S_1,\ldots$ is a martingale with respect to the sequence $X_0,X_1,\ldots$ if, for all $n\geq 0$, $\Exp{|S_t|}\leq \infty$ and $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.

% \begin{itemize}
% %\item $S_t$ is a function of $X_0,\ldots,X_n$;
% \item $\Exp{|S_t|}\leq \infty$; 
% \item $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.
% \end{itemize}
 \end{definition}

Given a martingale sequence $S_0,S_1, \ldots,S_y$, the sequence
% we refer to the martingale obtained as:
\begin{equation*}
Z_i = S_i - S_{i-1},\quad \mbox{for}\ i\geq 1
\end{equation*}
is the ``\emph{Difference martingale}'' (or ``\emph{Martingale Difference Sequence}'') corresponding to $S_0, S_2\ldots$. 
% Note that, as $S_0,\ldots,S_t$ is a martingale, $\Exp{|Z_t|}\leq \infty$ and for all $i = 1,\ldots,t$ we have $\Exp{Z_i|S_i,\ldots,Z_0} = 0$.

Finally, given a function of $n$ random variables
$Y=f(X_1,\ldots,X_n)$, such that $\Exp{|Y|}\leq \infty$, the sequence 
\begin{equation*}
C_i =\Exp{Y|X_i = x_i,\ldots,X_0= x_0},~~~i=0,\ldots,n
\end{equation*}
is a martingale, referred to as ``\emph{Doob martingale}''~\cite{mitzenmacher2017probability}. Note that $C_0=\Exp{Y}$ and
$C_n=f(x_1,\ldots, x_n)$.

In our work, we introduce the use of the Martingale Central Limit Theorem (MCLT), as an alternative way to obtain a bound on the generalization error. In particular, we apply the following version of MCLT~\footnote{Formally the asymptotic is defined on a triangle array where rows are samples of growing sizes. We also assume that all expectations are well defined in the corresponding filtration.}:
%In the previous section we have discussed how it is possible to bound the generalization error by means of the Rademacher Average (Theorem ), and how to obtain an estimate o. Both these result are achieved by applying McDiarmid's inequality. While correct, the bounds obtained using this approach often appear to be overly conservative. In this section we introduce the use of the Martingale Central Limit Theorem (MCLT), as an alternative way to obtain a bound on the generalization error.
\begin{theorem}{~\cite{hall2014martingale}[Corollary 3.2]}
Let $Z_0,Z_1,\dots$ be a difference martingale with bounded absolute increments. 
Assume that (1)  
$\sum_{i=1}^n Z_i^2 \stackrel{p}\rightarrow V^2$, for a finite $V>0$; and (2) $\Exp{\max_i Z^2_i}\leq M <\infty$,
then $\sum_{i=1}^n Z_i/\sqrt{\sum_{i=1}^n \Exp{Z_i^2}}$ converges in distribution to $N(0,1)$.
\end{theorem}
%Our algorithm estimates the Rademacher complexity ${R}_m^{{\cal F}_{k+1}}$ by the empirical Rademacher complexity ${R}_{\bar{x}}^{{\cal F}_{k+1}}$. The empirical Rademacher complexity ${R}_{\bar{x}}^{{\cal F}_{k+1}}$ is estimated using $\ell$ independent Rademacher vectors 
%$\bar{\sigma}_1,\dots, \bar{\sigma}_\ell$, each composed of $m$ independent Rademacher  random variables:
In order to actually use the Rademacher Average bound, we need to estimate ${R}_m^{{\cal F}_{k+1}}$ using our sample $\bar{x}$. Let $\bar{\sigma}_1,\dots, \bar{\sigma}_\ell$ be
 $\ell$ independent vectors each composed by $m$ Rademacher  random variables (i.e., $\bar{\sigma}_j = \sigma_{j,1}\sigma_{i,2}\ldots\sigma_{j,m}$ ). We will estimate  ${R}_m^{{\cal F}_{k+1}}$ as
\begin{equation}\label{eq:radestimate}
\tilde{R}_{\bar{x},\ell}^{{\mathcal F}_{k+1}}=\frac{1}{\ell}\sum_{j=1}^\ell\sup_{f\in {\cal F}}\frac{1}{m}\sum_{i=1}^m f(x_i)\sigma_{j,i} .
\end{equation}
 
Clearly $\Expe{\bar{x},\bar{\sigma_1},\dots,\bar{\sigma}_\ell} {\tilde{R}_{\bar{x},\ell}^{{\mathcal F}_{k+1}}}=R^{{\cal F}_{k+1}}_m$.

\begin{theorem}\label{thm:mclrad}
	\begin{equation*}
		\lim_{m\rightarrow \infty} \Prob{\maxErr{\mathcal{F}, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}> \epsilon}\geq 1 - \Phi\left(\frac{2\epsilon \sqrt{\ell m}}{\sqrt{\ell +4\sqrt{\ell} +20}}\right).
	\end{equation*}
\end{theorem}
\begin{proof}
	Consider the Doob maringale for the function $\maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{{\mathcal F}}_{\bar{x}}$:
	\begin{equation*}
		C_i = \Exp{\maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_i},
	\end{equation*}
where for $1\leq i\leq m$,
$Y_i = X_i$, and the remaining $m\ell$ $Y_i$ are the iid Rademacher random variables in the $\ell$ vectors, (i.e., $Y_{j(m)+i}= \sigma_{j,i}$, for $1\leq j\leq \ell$ and $1\leq i \leq m$).
%To apply the MCLT we define a difference martingale with respect to Doob martingale for the function $G(\bar{x}, \bar{\sigma}_1,\dots, \bar{\sigma}_\ell)$. In order to simplify the notation let $Y_1,\dots,Y_m=x_1,\dots,x_m$, and for $m+1\leq i \leq (\ell+1)m$ let $Y_i$ be the $i \textrm{mod } m $ Rademacher variable entry in the $\lfloor i/m \rfloor$ Rademacher vector. Our Doob martingale is defined for $0\leq i\leq (k+1)n$ as 
Further, let us define the corresponding martingale difference sequence
$$Z_i=C_i-C_{i-1}.$$
Note that for each $i\in\{1,\ldots,m(\ell+1)\}$, due to linearity of expectation, we have:
\begin{align*}
Z_i &= A_i - 2B_i;\\
A_i &= \Exp{\maxErr{\mathcal{F},\bar{x}}|Y_1,\ldots Y_i}- \Exp{\maxErr{\mathcal{F},\bar{x}}|Y_1,\ldots Y_{i-1}};\\
B_i &= \Exp{\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_{i}}- \Exp{\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_{i-1}}.
\end{align*}
In order to apply the Martingale Central Limit Theorem we need to bound the values $\Exp{Z_i^2}$. Given our definition of the difference martingale $Z_i$,  we have that for every $i$, $\Exp{Z_i}=\Exp{A_i}=\Exp{B_i}=0$, and thus $\Exp{Z_i^2}=\Var{Z_i}\leq \Var{A_i}+4\Var{B_i} + 4\sqrt{\Var{A_i}\Var{B_i}}$:
\begin{itemize}
\item $1\leq i\leq m$: as is our setting $\forall x\in \mathcal{X}$ and $\forall f \in \mathcal{F}$, $f(x) \in [0,1]$, changing the value of any of the $m$ points in $\bar{x}$ can change $f(\bar{x})$ by at most $1/m$. Thus, by applying Popoviciu's inequality~\cite{popoviciu1935equations}, we have: $\Var{A_i}\leq (b-a)^2/(4m^2)$. Following the same reasoning, and by noting that (a) we are considering the expectation over the unassigned values of the Rademacher random variables, and (b) we are averaging over the values obtained using $\ell$ iid vectors of Rademacher random variables, we have: $\Var{B_i}\leq 1/(4m^2\ell)$. We can thus conclude:
 \begin{align*}
	\Exp{Z_i^2}=\Var{Z_i} &\leq \frac{1}{4m^2}+\frac{4}{4\ell m^2} + 4\sqrt{\frac{1}{4m^2}\frac{1}{4\ell m^2}}\\
	&\leq \frac{\ell + 4 +4\sqrt{\ell}}{4m^2\ell}.
 \end{align*}

\item $m < i\leq m(\ell +1)$: Note that changing the value of any of the Rademacher random variables does not change the value of $\maxErr{\mathcal{F},\bar{x}}$, hence $\Var{A_i}=\Exp{A_i^2} = 0$. Note that, given a fixed values for the the random corresponding to the points in $\bar{x}$,  that changing the value of one Rademacher Random variables can change the value of $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ by at most $2/\ell m$. Therefore by applying Popoviciu's inequality~\cite{popoviciu1935equations}:
\begin{align*}
	\Exp{Z_i^2}=\Var{Z_i} = 4\Var{B_i} \leq \frac{4}{m^2 \ell^2}
\end{align*}
\end{itemize}
Applying the MCLT we have that  as $m$ goes to infinity $\sum_{i=1}^{\ell (m+1)} Z_i/\sqrt{\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2}}$ converges in distribution to $N(0,1)$, and thus $\sum_{i=1}^{\ell (m+1)} Z_i$ converges to  $N(0,\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2})$. Hence we have:
\begin{align*}
\lim_{m\rightarrow\infty} \Prob{\sum_{i=1}^{\ell (m+1)} Z_i > \epsilon} &< 1 -\Phi\left(\frac{\epsilon}{\sqrt{\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2}}}\right).
\end{align*}
By linearity of expectation, and by applying Theorem~\ref{th:Ra}:
\begin{align*}
	\sum_{i=1}^{\ell (m+1)} Z_i &= \maxErr{\mathcal{F},\bar{x}} - \Exp{\maxErr{\mathcal{F},\bar{x}}} -2\left(\tilde{R}^{\mathcal F}_{\bar{x},\ell} - R^{\mathcal F}_{m}\right)\\
	&\geq \maxErr{\mathcal{F},\bar{x}} - 2R^{\mathcal F}_{m} -2\left(\tilde{R}^{\mathcal F}_{\bar{x},\ell} - R^{\mathcal F}_{m}\right);\\
	&\geq \maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{\mathcal F}_{\bar{x},\ell};
\end{align*} 
Further,
\begin{align*}
\sum_{i=1}^{m (\ell+1)}\Exp{Z_i^2} &= \sum_{i=1}^{m}\Exp{Z_i^2} + \sum_{i=m+1}^{m (\ell+1)} \Exp{Z_i^2};\\
& \leq m\frac{\ell + 4 +4\sqrt{\ell}}{4m^2\ell} + m\ell\frac{4}{m^2 \ell^2};\\
&\leq \frac{\ell + 4\sqrt{\ell}+20}{4m\ell}	
\end{align*} 
% $$\sum_{i=1}^{m (\ell+1)}\Exp{Z_i^2} = \sum_{i=1}^{m}\Exp{Z_i^2} + \sum_{i=m+1}^{m (\ell+1)} \Exp{Z_i^2}$$
% $$ \leq m\frac{\ell + 4 +4\ell}{4m^2\ell} + m\ell\frac{4}{m^2} 
% \leq \frac{\ell + 4\sqrt{\ell}+20}{4m\ell}.$$
% \end{align*} 
The statement follows.
\end{proof}

An even tighter bound can be obtained by splitting the analysis into two parts: (a) bound on the generalization error, and (b) bound on the quality of the \Rade estimation. We present these result in Appendix~\ref{app:mcltbound2}. 
% The bounds obtained using by application of the MCLT are crucially different from those achieved using McDiarmids's inequality (Section 3) as they characterize the asymptotic behavior of the quantities being analyzed. This allows to obtain a much tighter estimate.
Our application of the MCLT to estimating the Rademacher complexity gives significantly better results than the bounds obtained by applying McDiarmid inequality to similar computations (see Figures~\ref{fig:exp1}, \ref{fig:exp2} , and \ref{fig:exp4}).
The significant improvement in using the MCLT instead of McDiarmid inequality based bounds is not due just to fact that the MCLT is an asymptotic result. A more significant difference that while the bound on the \Rade approximation obtained using the MCLT depends on the second moment of the variation of the value of the function being considered (i.e., $\Exp{Z_i}$), while the bound obtained McDiarmid's inequality depends on the maximum variation of such value (i.e., $\max_{z\in\mathcal{X}, f\in \mathcal{F}} Z_i$).
In particular, this fact allows to better characterize the improvement obtained in the quality of the estimate  using  multiple vectors of Rademacher random variables.
% Note that the proposed approach which uses the MCLT the quality of the obtained estimates depends on a bound on the variance of $Z_i$, that is of the change of the value of the function  $\maxErr{\mathcal{F}, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}$ when the value of one of the $m$ random variables corresponding to points in $\bar{x}$ and to the $\ell m$ Rademacher random variables used to compute $\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}$ changes.The usual bounds obtained using McDiarmid approach, depend instead on a bound on the actual value of $Z_i$. This fact allows to better characterize the improvement obtained in the quality of the estimate  using  multiple vectors of Rademacher random variables, and is one of the main reasons due to which the MCLT bound is considerably tighter than bounds based on McDiarmid.
By exploiting this same fact, we show that using an appropriate application of Bernstein's inequality for martingales, it is indeed possible to obtain a rigorous, finite sample size bound tighter than the ones achieved using McDiarmid's inequality (see Appendix~\ref{app:bernbound}).



==> 03n_boundinggenerror_old.tex <==
%\section{Generalization error bounds with \Rade{}}\label{sec:bound}
\subsection{Tight bounds on \Rade{} estimate}\label{sec:bound}
Given a finite size sample $\bar{x}\sim \mathcal{D}^m$ and $\ell$ independent Rademacher vectors  $\bar{\sigma}_1,\dots, \bar{\sigma}_\ell$, each composed of $m$ independent Rademacher random variables (i.e., $\bar{\sigma}_j = \sigma_{j,1}\sigma_{i,2}\ldots\sigma_{j,m}$ ), we estimate ${R}_m^{\mathcal{F}_k}$ with
%
%In order to actually use the Rademacher Complexity results for a given hypothesis class $\mathcal{F}$, it is necessary to  estimate ${R}_m^{{\cal F}}$ using a given, finite size, sample $\bar{x}\sim \mathcal{D}^m$. Let $\bar{\sigma}_1,\dots, \bar{\sigma}_\ell$ be $\ell$ independent vectors each composed each by $m$ independent Rademacher random variables (i.e., $\bar{\sigma}_j = \sigma_{j,1}\sigma_{i,2}\ldots\sigma_{j,m}$ ). Consider the estimate of  ${R}_m^{{\cal F}}$ computed as:
\begin{equation}\label{eq:radestimate}	\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}=\frac{1}{\ell}\sum_{j=1}^\ell\sup_{f\in \mathcal{F}_k}\frac{1}{m}\sum_{i=1}^m f(x_i)\sigma_{j,i}.
\end{equation}
Clearly, $\Expe{\bar{x},\bar{\sigma_1},\dots,\bar{\sigma}_\ell} {\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}}=R^{\mathcal{F}_k}_m$.
To bound the error $R^{\mathcal{F}_k}_m- \tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$, we model the process as a \emph{Doob martingale} (\citealp[Chapter 13.1]{mitzenmacher2017probability}) as follows: 
$$C_i=E[R^{\mathcal{F}_k}_m- \tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}~|~Y_1,\dots,Y_i]~~ \mbox{for}~i=0,\dots,m(\ell+1),$$
where the $Y_1,\ldots,Y_{m(\ell+1)}$ are the random variables that determinate the value of the estimate $\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$. The first $m$ variables $Y_i$'s correspond to the values of the sample $\bar{x}$, i.e. for $1\leq i\leq m$, $Y_i=X_i$, and the remaining $m\ell$ $Y_i$'s correspond to the Rademacher random variables,  $Y_i= \sigma_{\lfloor i/m \rfloor, i- \lfloor i/m \rfloor}$. It is easy to verify that $C_0=0$, and $C_{m(\ell+1)}= R^{\mathcal{ F}}_m- \tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$.

Next, we define a \emph{martingale difference sequence} $Z_i=C_i-C_{i-1}$ with respect to the martingale $C_0, C_1, \dots C_{m(\ell+1)}$, and note that $\sum_{t=1}^{m(\ell+1)} Z_t=C_{m(\ell+1)} = R^{\mathcal{F}_k}_m- \tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$.

%In order to obtain guarantees on the quality of the approximation (i.e., a bound on $|\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}-R^{{\cal F}}_m|$), we analyze the estimation process of the Rademacher complexity as a \emph{Doob martingale}. We will use the following basic definitions:
%% \paragraph{Martingales}
%% We introduce here some basic concepts relative to martingales which we will use in our derivations.
%\begin{definition}{\cite{mitzenmacher2017probability}}
%A sequence of random variables $S_0,S_1,\ldots,S_t$ is a martingale with respect to the sequence of random variables $X_0,X_1,\ldots,X_t$ if, for all $t\geq 0$, $\Exp{|S_t|}\leq \infty$ and $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.
%% \begin{itemize}
%% %\item $S_t$ is a function of $X_0,\ldots,X_n$;
%% \item $\Exp{|S_t|}\leq \infty$; 
%% \item $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.
%% \end{itemize}
% \end{definition}
%Given a martingale $S_0,S_1, \ldots,S_t$, the sequence $Z_i = S_i - S_{i-1}$, for $i\geq 1$ is referred as the ``\emph{Martingale Difference Sequence}'' corresponding to $S_0, S_1\ldots,S_t$. 
%% Note that, as $S_0,\ldots,S_t$ is a martingale, $\Exp{|Z_t|}\leq \infty$ and for all $i = 1,\ldots,t$ we have $\Exp{Z_i|S_i,\ldots,Z_0} = 0$.
%Finally, given a function of $n$ random variables
%$Y=f(X_1,\ldots,X_n)$, such that $\Exp{|Y|}\leq \infty$, the sequence 
%\begin{equation*}
%C_i =\Exp{Y|X_i = x_i,\ldots,X_0= x_0},~~~i=0,\ldots,n
%\end{equation*}
%is a martingale, referred as ``\emph{Doob martingale}''~\cite{mitzenmacher2017probability}, with $C_0=\Exp{Y}$ and
%$C_n=f(x_1,\ldots, x_n)$.
%
\paragraph{Application of Bernstein's Inequality for Martingales} Our first bound builds on Bernstein's Inequality for Martingales (BIM). We use the following version due to  Freedman~\cite{freedman1975tail}, as presented in~\cite{dzhaparidze2001bernstein} and adapted to one-sided error.
%We characterize the quality of the approximation of the \Rade{} ${R}_m^{{\cal F}}$ given by $\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}$ using a novel application of 
\begin{theorem}\label{thm:bernmain}{\cite{dzhaparidze2001bernstein,  freedman1975tail}}
Let $Z_1,\ldots,Z_t $ be a martingale difference sequence with respect to a certain filtration $\{\mathscr{F}_i\}_{i=0,\ldots,t}$. 

Thus, $\Exp{Z_i|\mathscr{F}_{i-1}} = 0$ for $i=1,\ldots,t$. The process $\sum_{i=1}^t Z_i$ is thus a martingale with respect to this filtration. Further, assume that $|Z_i|\leq a$ for $i=1,\ldots,t$, and that the conditional variance $\sum_{i=1}^t \Exp{Z_i^2}\leq L$. For $\epsilon \in (0,1)$, we have:
\begin{equation}
\Prob{\sum_{i=1}^t Z_i>\epsilon}\leq e^{-\frac{\epsilon^2}{2L+2a\epsilon/3}}.
\end{equation}
\end{theorem}
Note that the bound presented here is slightly different from the one in~\cite{freedman1975tail} as for our purposes we only require a one-sided bound.
 
A careful analysis of $E[Z_i^2]$ in our application allows us to obtain a significantly stronger bound than the one obtained using McDiarmid's Inequality~\cite{Barlett02,ShalevSBD14}, which depends on the maximum variation of the martingale. In particular, (in Appendix~\ref{app:bernbound}\label{lem:bernrade}) we prove:
%We now use this result to characterize the distribution of $R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x}}$.
\begin{theorem}% {Proof in Appendix~\ref{app:bernbound}}
Given a sample $\bar{x}\sim \mathcal{D}^m$, a family of functions $\mathcal{F}_k$ which take values in $[0,1]$,  $\ell$ independent vectors of Rademacher random variables, and $\epsilon, \delta \in (0,1)$, we have: 
\label{lem:bernrade}
\begin{equation}
\label{eq:radestimate1}
\Prob{R^{\mathcal{F}_k}_{m}- \tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}>\epsilon}\leq  e^{- \frac{6m \ell \epsilon^2}{15+ 8\ell \epsilon}}.
 \end{equation}
\end{theorem}

Note that for a sufficiently large (constant) $\ell$, the term $6\epsilon \ell$ dominates the denominator of the exponent in the right hand side of~\eqref{eq:radestimate1}, giving
%thus $\textrm{Pr}(R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}) \in \mathcal{O}\left( e^{\epsilon m} \right)$. That is, 
a \emph{fast rate of convergence} for the estimate. Our estimate fully characterizes the benefit achieved using  multiple independent vectors of Rademacher random variables in estimating $\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}$. 
See Appendix~\ref{app:comparison} for a comparison to the bound achieved by applying McDiarmid's Inequality to similar estimates (as discussed in Appendix~\ref{app:refinedmcdia}).

%Our application of the BIM for the analysis of the quality of the approximation of the \Rade{} leads to much tighter bounds than those achievable by applying McDiarmid's Inequality to similar computations (see Figures~\ref{fig:exp1}, \ref{fig:exp2} , and \ref{fig:exp4}).
%This is mostly due to the fact that while the bound obtained McDiarmid's Inequality depends on the maximum variation of $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ which may be caused by changing one of the samples in $\bar{x}$ (i.e., $\max_{z\in\mathcal{X}, f\in \mathcal{F}} Z_i$), when using the BIM one consider instead the second moment of such variation. In particular, this using the BIM allows to fully characterize the benefit achieved using  multiple independent vectors of Rademacher random variables in the computation of the estimate $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$. A detailed analysis of the bounds achievable using Mc Diarmid's inequality for $R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}$ is presented in Appendix~\ref{app:refinedmcdia}.

Combining the results of Theorem~\ref{lem:bernrade}, Lemma~\ref{th:Ra}, and Lemma~\ref{th:Ra2} using the union bound, we obtain a tight empirical bound on $\maxErr{\mathcal{F}_k,\bar{x}}$ (proof in Appendix~\ref{app:bernbound}).
\begin{theorem}\label{thm:bernradetot}Given a sample $\bar{x}\sim \mathcal{D}^m$, a family of functions $\mathcal{F}_k$ which take values in $[0,1]$,  $\ell$ independent vectors of Rademacher random variables, and $\epsilon, \delta \in (0,1)$, we have:
% $
% 	\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}+ \epsilon_1+2\epsilon_2}<e^{-2m\epsilon_1^2}+e^{-\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}}.
% $
% \begin{equation}
% 	\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}+ \epsilon_1+2\epsilon_2}<e^{-2m\epsilon_1^2}+e^{-\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}}.
% \end{equation}
\small
\begin{equation}
\Prob{\Psi (\mathcal{F}_k,\bar{x}) > 2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}+ \epsilon}  
< \min_{\alpha\in(0,\epsilon)}  e^{-2m(\epsilon-\alpha)^2}+e^{-\frac{3m \ell \alpha^2}{30+ 8\ell \alpha}}.
\end{equation}
\normalsize
\end{theorem}
\subsection{Application of the Martingale Central Limit Theorem}\label{sec:mclt}
In practical applications, one may prefer the standard practice in statistics of applying central limit asymptotic bounds. We develop here a bound based on the Martingale Central Limit Theorem (MCLT).  Our experimental results in Section~\ref{sec:exper} show that the bound obtained using the MCLT is more powerful while still preserving statistical validity. Further comparison of the bounds is presented in Appendix~\ref{app:comparison}.

%While allowing for a tight analysis of the generalization error for the finite sample case, in several practical scenarios, especially when dealing with a small sample, the previously discussed bounds may still be overly conservative.
We adapt the following version of the MCLT~\footnote{Formally, the asymptotic is defined on a triangle array, where rows are samples of growing sizes. We also assume that all expectations are well-defined in the corresponding filtration.}:
%In the previous section we have discussed how it is possible to bound the generalization error by means of the Rademacher Average (Theorem ), and how to obtain an estimate o. Both these result are achieved by applying McDiarmid's Inequality. While correct, the bounds obtained using this approach often appear to be overly conservative. In this section we introduce the use of the Martingale Central Limit Theorem (MCLT), as an alternative way to obtain a bound on the generalization error.
\begin{theorem}[\emph{Corollary 3.2,} \citealp{hall2014martingale}]
Let $Z_0,Z_1,\dots$ be a difference martingale with bounded absolute increments. 
Assume that (1)  
$\sum_{i=1}^n Z_i^2 \stackrel{p}\rightarrow V^2$ for a finite $V>0$, and (2) $\Exp{\max_i Z^2_i}\leq M <\infty$,
then $\sum_{i=1}^n Z_i/\sqrt{\sum_{i=1}^n \Exp{Z_i^2}}$ converges in distribution to $N(0,1)$.
\end{theorem}

When applying the MCLT, there is no advantage in bounding separately $\maxErr{\mathcal{F}_k, \bar{x}}-2R^{\mathcal{F}_k}_{m}$ and    $2R^{\mathcal{F}_k}_{m}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$. Instead, we compute a bound on the distribution of $\maxErr{\mathcal{F}_k, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}$ by analyzing the \emph{Doob supermartingale}
$$C_i=E[\maxErr{\mathcal{F}_k, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}~|~Y_1,\dots,Y_i]$$
for $i=0,\dots,m(\ell+1)$,  with respect to the same $Y_1,\dots, Y_{m(\ell+1)}$ defined as in Section 3.1.

As in the finite sample case, the following theorem relies on a careful analysis of $\Exp{Z_i^2}$ for the martingale difference sequence $Z_i =C_i-C_{i-1}$ (proof in Appendix~\ref{app:mcltbound2}).
\begin{theorem}\label{thm:mclrad}Given a sample $\bar{x}\sim \mathcal{D}^m$, a family of functions $\mathcal{F}_k$ which take values in $[0,1]$,  $\ell$ independent vectors of Rademacher random variables, and $\epsilon, \delta \in (0,1)$, we have: 
\small
	\begin{equation*}
		\lim_{m\rightarrow \infty} \Prob{\maxErr{\mathcal{F}_k, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}> \epsilon \frac{\sqrt{\ell +4\sqrt{\ell} +20}}{2 \sqrt{\ell m}}}< 1 - \Phi\left(\epsilon \right). 
	\end{equation*}
\normalsize
Where $\Phi(x)$ denotes the cumulative distribution function for the standard normal distribution.
\end{theorem}
%While it is not possible to compare directly the tightness of the \emph{asymptotic} bound in Theorem~\ref{thm:mclrad} with that of \emph{finite sample} bounds such as the one in Theorem~\ref{thm:bernradetot}, this result is of great interest in many practical scenarios as it allows for a much tighter characterization of the generalization error.
%%
%%
Due to its asymptotic nature, it is not possible to compare directly the tightness of the bound in Theorem~\ref{thm:mclrad} with that of finite sample bounds such as the one in Theorem~\ref{thm:bernradetot}. Still, this bound is of great interest in many practical scenarios as it allows for a much tighter bound for the generalization error.
%%
%
%The use of asymptotic bounds is common practice in classical statistical tests (e.g., the \emph{student t\- test}, the \emph{z\- test}). Further, 

==> 03nal_boundinggenerror.tex <==
\section{Bounding the generalization error using Bernstein's inequality for Martingales}\label{app:bernbound}

In order to actually use the Rademacher Complexity results for a given hypothesis class $\mathcal{F}$, it is necessary to  estimate ${R}_m^{{\cal F}}$ using a given, finite size, sample $\bar{x}$. Let $\bar{\sigma}_1,\dots, \bar{\sigma}_\ell$ be
 $\ell$ independent vectors each composed each by $m$ independent Rademacher  random variables (i.e., $\bar{\sigma}_j = \sigma_{j,1}\sigma_{i,2}\ldots\sigma_{j,m}$ ). We will estimate  ${R}_m^{{\cal F}_{k+1}}$ as:
\begin{equation}\label{eq:radestimate}
\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}=\frac{1}{\ell}\sum_{j=1}^\ell\sup_{f\in {\cal F}}\frac{1}{m}\sum_{i=1}^m f(x_i)\sigma_{j,i} .
\end{equation}
 
By linearity of expectation, we clearly have: $\Expe{\bar{x},\bar{\sigma_1},\dots,\bar{\sigma}_\ell} {\tilde{R}_{\bar{x},\ell}^{\mathcal F}}=R^{\cal F}_m$.

In order to obtain guarantees on the quality of the approximation (i.e., a bound on $|\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}-R^{{\cal F}}_m|$), we analyze the estimation process of the Rademacher complexity as a \emph{Doob martingale}. We will use the following basic definitions:
% \paragraph{Martingales}
% We introduce here some basic concepts relative to martingales which we will use in our derivations.
\begin{definition}{\cite{mitzenmacher2017probability}}
A sequence of random variables $S_0,S_1,\ldots,S_t$ is a martingale with respect to the sequence $X_0,X_1,\ldots,X_t$ if, for all $n\geq 0$, $\Exp{|S_t|}\leq \infty$ and $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.

% \begin{itemize}
% %\item $S_t$ is a function of $X_0,\ldots,X_n$;
% \item $\Exp{|S_t|}\leq \infty$; 
% \item $\Exp{S_{t+1}|X_0,\ldots,X_t} = S_t$.
% \end{itemize}
 \end{definition}

Given a martingale $S_0,S_1, \ldots,S_t$, the sequence $Z_i = S_i - S_{i-1}$, for $i\geq 1$ is referred as the ``\emph{Martingale Difference Sequence}'' (or, the ``\emph{Difference martingale}'') corresponding to $S_0, S_2\ldots,S_t$. 
% Note that, as $S_0,\ldots,S_t$ is a martingale, $\Exp{|Z_t|}\leq \infty$ and for all $i = 1,\ldots,t$ we have $\Exp{Z_i|S_i,\ldots,Z_0} = 0$.
Finally, given a function of $n$ random variables
$Y=f(X_1,\ldots,X_n)$, such that $\Exp{|Y|}\leq \infty$, the sequence 
\begin{equation*}
C_i =\Exp{Y|X_i = x_i,\ldots,X_0= x_0},~~~i=0,\ldots,n
\end{equation*}
is a martingale, referred to as ``\emph{Doob martingale}''~\cite{mitzenmacher2017probability}. Note that $C_0=\Exp{Y}$ and
$C_n=f(x_1,\ldots, x_n)$.

In this section we discuss a novel application of Bernstein's Inequality for Martingales for characterizing the quality of the approximation of the \Rade ${R}_m^{{\cal F}}$. In particular, in this work we refer to a version of this result due to Freedman~\cite{freedman1975tail}:

\begin{theorem}\label{thm:bernmain}
Let $Z_1,Z_2,\ldots $ be a martingale difference sequence with respect to a certain filtration $\{\mathscr{F}_i\}_{i=0,1,\ldots}$. Thus $\Exp{Z_i|\mathscr{F}_{i-1}} = 0$ for every $i$. The process $\sum_{i=1}^t Z_i$ is thus a martingale with respect to this filtration. Furthermore assume that $|Z_i|\leq a$ for an all $i $ and that the conditional variance of $\sum_{i=1}^t Z_i$ is bounded from above by $L$. We have:
\begin{equation}
\Prob{\sum_{i=1}^t Z_i>\epsilon}\leq e^{-\frac{\epsilon^2}{2L+2a\epsilon/3}}.
\end{equation}
\end{theorem}

Note that the bound presented here is slightly different from the one in~\cite{freedman1975tail} as for our purposes we only require a one-sided bound.
 
We now use this result to characterize the distribution of $R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x}}$.

\begin{lemma}\label{lem:bernrade}
\begin{equation}
\Prob{R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}>\epsilon_2}\leq e^{-\frac{\epsilon^2}{\frac{5}{2\ell m }+\frac{4\epsilon}{3m}}}.
 \end{equation}
\end{lemma}
\begin{proof}
By definition, $\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}$ is a function of $\ell(m+1)$ independent random variables $Y_i$. For the simplicity purposes, assume $Y_i = X_i$ for $1\leq i \leq m$, and the remaining $Y_i$ are the $\ell m$ iid Rademacher Random Variables which compose the $\ell$ vectors of Rademacher random variables (i.e., $Y_{j(m)+i}= \sigma_{j,i}$, for $1\leq j\leq \ell$ and $1\leq i \leq m$).
Let us define the Doob martingale:
\begin{equation}
C_i = \Exp{\tilde{R}^{\mathcal F}_{\bar{x},\ell}|Y_1,\ldots,Y_i}
\end{equation}
Let us consider the corresponding difference martingale $Z_i = C_{i+1}-C_{i}$. Note that by the definition of $Z_i$, $\Exp{Z_i}=0$ for every $i=1,\ldots,m$.  In order apply Bernstein's inequality we need to Bound the values of  values of $\Exp{Z_i^2}$ we shall consider separately the cases for for $1\leq i\leq m$ and $m<i\leq \ell (m+1)$:
\begin{itemize}
\item $1\leq i\leq m$: as is our setting $\forall x\in \mathcal{X}$ and $\forall f \in \mathcal{F}$, $f(x) \in [0,1]$, changing the value of any of the $m$ points in $\bar{x}$ can change $f(\bar{x})$ by at most $1/m$. Thus, by applying Popoviciu's inequality~\cite{popoviciu1935equations}, we have: $\Var{Z_i}\leq 1/(4m^2)$. Following the same reasoning, and by noting that (a) we are considering the expectation over the unassigned values of the Rademacher random variables, and (b) we are averaging over the values obtained using $\ell$ iid vectors of Rademacher random variables, we have: $\Var{Z_i}\leq 1/(4m^2\ell)$.
\item $ i> m$: note that changing the value of one Rademacher Random variable can change the value of $\tilde{R}^{\mathcal F}_{\bar{x},j}$ by at most $2/\ell m$.
% In particular, if changed, the value can change by either $1/\ell m$ or $2/\ell m$. 
By applying Popoviciu's inequality~\cite{popoviciu1935equations}, we have $\Exp{Z_i^2}=\Var{Z_i}\leq \frac{1}{4m^2}$ for $m<i\leq m(\ell+1)$.
\end{itemize}
By linearity of expectation, $\sum_{i=1}^{\ell (m+1)} Z_i = \tilde{R}^{\mathcal F}_{\bar{x},\ell} - R^{\mathcal F}_{m}$. Further, we have $\sum_{i=1}^{\ell (m+1)} Z_i^2 \leq 5/4\ell m$, and that $|Z_i|<2/m$ for all $i\geq 1$.
%By applying the MCLT we therefore have:
%\begin{align*}
%&\lim_{m\rightarrow\infty} \Prob{\frac{2\sqrt{\ell m}}{\sqrt{5}}\left(\tilde{R}^{\mathcal F}_{\bar{x}} - R^{\mathcal F}_{\bar{x}}\right)>\epsilon}\\&\qquad\leq  \Prob{\tilde{R}^{\mathcal F}_{\bar{x}} - R^{\mathcal F}_{\bar{x}}> \frac{2\sqrt{\ell m}}{\sqrt{5}} \epsilon}\leq 1-\Phi(\frac{2\sqrt{\ell m}}{\sqrt{5}}\epsilon).
% \end{align*}
The statement follows by applying Theorem~\ref{thm:bernmain}. 
\end{proof}

Our application of the Bernstein's inequality for the analysis of the quality of the approximation of the Rademacher complexity leads to much tighter bounds than those achievable by applying McDiarmid's inequality to similar computations (see Figures~\ref{fig:exp1}, \ref{fig:exp2} , and \ref{fig:exp4}).
This is mostly due to the fact that while the bound on the \Rade approximation obtained using Bernstein's inequality for martingales depends on the second moment of the variation of the value of the function being considered (i.e., $\Exp{Z_i}$), while the bound obtained McDiarmid's inequality depends on the maximum variation of such value (i.e., $\max_{z\in\mathcal{X}, f\in \mathcal{F}} Z_i$).
In particular, this fact allows to better characterize the improvement obtained in the quality of the estimate  using  multiple vectors of Rademacher random variables. For a detailed analysis of the bounds achievable using Mc Diarmid's inequality for $R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}$ we refer the reader to Appendix~\ref{app:refinedmcdia}.

We can bound the generalization error $\maxErr{\mathcal{F},\bar{x}}$ in terms of the estimated \Rade{} of $\mathcal{F}$ as by combining the results of Theorems~\ref{th:Ra} and~\ref{thm:mainrade}, with Lemma Lemmas~\ref{lem:mcltgen}-~\ref{lem:bernrade}:
\begin{theorem}
\begin{equation}
	\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}^{\cal F}_m+ \epsilon_1+2\epsilon_2}<e^{-2m\epsilon_2^2}+e^{-\frac{\epsilon^2}{\frac{5}{2\ell m }+\frac{4\epsilon_2}{3m}}}.
\end{equation}
\end{theorem}

\subsection*{Bounding the generalization error using the Martingale Central Limit Theorhem}

While the previously discussed bound allow for a tight analysis of the generalization error for the finite sample case, in several practical scenarios, especially when dealing with a small sample, the obtained bounds may still result to be loose for practical use.

We introduce the use of the Martingale Central Limit Theorem (MCLT), as a way to obtain an alternative, asymptotic, bound on the generalization error. In particular, we apply the following version of MCLT~\footnote{Formally the asymptotic is defined on a triangle array where rows are samples of growing sizes. We also assume that all expectations are well defined in the corresponding filtration.}:
%In the previous section we have discussed how it is possible to bound the generalization error by means of the Rademacher Average (Theorem ), and how to obtain an estimate o. Both these result are achieved by applying McDiarmid's inequality. While correct, the bounds obtained using this approach often appear to be overly conservative. In this section we introduce the use of the Martingale Central Limit Theorem (MCLT), as an alternative way to obtain a bound on the generalization error.
\begin{theorem}{~\cite{hall2014martingale}[Corollary 3.2]}
Let $Z_0,Z_1,\dots$ be a difference martingale with bounded absolute increments. 
Assume that (1)  
$\sum_{i=1}^n Z_i^2 \stackrel{p}\rightarrow V^2$, for a finite $V>0$; and (2) $\Exp{\max_i Z^2_i}\leq M <\infty$,
then $\sum_{i=1}^n Z_i/\sqrt{\sum_{i=1}^n \Exp{Z_i^2}}$ converges in distribution to $N(0,1)$.
\end{theorem}
The MCLT allows us to characterize the distribution of $\maxErr{\mathcal{F}, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}$:
\begin{theorem}\label{thm:mclrad}
	\begin{equation*}
		\lim_{m\rightarrow \infty} \Prob{\maxErr{\mathcal{F}, \bar{x}}-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}}> \epsilon \frac{\sqrt{\ell +4\sqrt{\ell} +20}}{2 \sqrt{\ell m}}}\geq 1 - \Phi\left(\epsilon \right).
	\end{equation*}
\end{theorem}
\begin{proof}
	Consider the Doob maringale for the function $\maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{{\mathcal F}}_{\bar{x}}$:
	\begin{equation*}
		C_i = \Exp{\maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_i},
	\end{equation*}
where for $1\leq i\leq m$,
$Y_i = X_i$, and the remaining $m\ell$ $Y_i$ are the iid Rademacher random variables in the $\ell$ vectors, (i.e., $Y_{j(m)+i}= \sigma_{j,i}$, for $1\leq j\leq \ell$ and $1\leq i \leq m$).
%To apply the MCLT we define a difference martingale with respect to Doob martingale for the function $G(\bar{x}, \bar{\sigma}_1,\dots, \bar{\sigma}_\ell)$. In order to simplify the notation let $Y_1,\dots,Y_m=x_1,\dots,x_m$, and for $m+1\leq i \leq (\ell+1)m$ let $Y_i$ be the $i \textrm{mod } m $ Rademacher variable entry in the $\lfloor i/m \rfloor$ Rademacher vector. Our Doob martingale is defined for $0\leq i\leq (k+1)n$ as 
Further, let us define the corresponding martingale difference sequence
$$Z_i=C_i-C_{i-1}.$$
Note that for each $i\in\{1,\ldots,m(\ell+1)\}$, due to linearity of expectation, we have:
\begin{align*}
Z_i &= A_i - 2B_i;\\
A_i &= \Exp{\maxErr{\mathcal{F},\bar{x}}|Y_1,\ldots Y_i}- \Exp{\maxErr{\mathcal{F},\bar{x}}|Y_1,\ldots Y_{i-1}};\\
B_i &= \Exp{\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_{i}}- \Exp{\tilde{R}^{{\mathcal F}}_{\bar{x}}|Y_1,\ldots Y_{i-1}}.
\end{align*}
In order to apply the Martingale Central Limit Theorem we need to bound the values $\Exp{Z_i^2}$. Given our definition of the difference martingale $Z_i$,  we have that for every $i$, $\Exp{Z_i}=\Exp{A_i}=\Exp{B_i}=0$, and thus $\Exp{Z_i^2}=\Var{Z_i}\leq \Var{A_i}+4\Var{B_i} + 4\sqrt{\Var{A_i}\Var{B_i}}$:
\begin{itemize}
\item $1\leq i\leq m$: as is our setting $\forall x\in \mathcal{X}$ and $\forall f \in \mathcal{F}$, $f(x) \in [0,1]$, changing the value of any of the $m$ points in $\bar{x}$ can change $f(\bar{x})$ by at most $1/m$. Thus, by applying Popoviciu's inequality~\cite{popoviciu1935equations}, we have: $\Var{A_i}\leq (b-a)^2/(4m^2)$. Following the same reasoning, and by noting that (a) we are considering the expectation over the unassigned values of the Rademacher random variables, and (b) we are averaging over the values obtained using $\ell$ iid vectors of Rademacher random variables, we have: $\Var{B_i}\leq 1/(4m^2\ell)$. We can thus conclude:
 \begin{align*}
	\Exp{Z_i^2}=\Var{Z_i} &\leq \frac{1}{4m^2}+\frac{4}{4\ell m^2} + 4\sqrt{\frac{1}{4m^2}\frac{1}{4\ell m^2}}\\
	&\leq \frac{\ell + 4 +4\sqrt{\ell}}{4m^2\ell}.
 \end{align*}

\item $m < i\leq m(\ell +1)$: Note that changing the value of any of the Rademacher random variables does not change the value of $\maxErr{\mathcal{F},\bar{x}}$, hence $\Var{A_i}=\Exp{A_i^2} = 0$. Note that, given a fixed values for the the random corresponding to the points in $\bar{x}$,  that changing the value of one Rademacher Random variables can change the value of $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ by at most $2/\ell m$. Therefore by applying Popoviciu's inequality~\cite{popoviciu1935equations}:
\begin{align*}
	\Exp{Z_i^2}=\Var{Z_i} = 4\Var{B_i} \leq \frac{4}{m^2 \ell^2}
\end{align*}
\end{itemize}
Applying the MCLT we have that  as $m$ goes to infinity $\sum_{i=1}^{\ell (m+1)} Z_i/\sqrt{\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2}}$ converges in distribution to $N(0,1)$, and thus:
\begin{align*}
\lim_{m\rightarrow\infty} \Prob{\sum_{i=1}^{\ell (m+1)} Z_i \left(\sqrt{\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2}}\right)^{-1} > \epsilon} &< 1 -\Phi\left(\epsilon\right),\\
\lim_{m\rightarrow\infty} \Prob{\sum_{i=1}^{\ell (m+1)} Z_i > \epsilon\sqrt{\sum_{i=1}^{m (\ell+1)} \Exp{Z_i^2}}} &< 1 -\Phi\left(\epsilon\right),\\
\end{align*}
By linearity of expectation, and by applying Theorem~\ref{th:Ra}:
\begin{align*}
	\sum_{i=1}^{\ell (m+1)} Z_i &= \maxErr{\mathcal{F},\bar{x}} - \Exp{\maxErr{\mathcal{F},\bar{x}}} -2\left(\tilde{R}^{\mathcal F}_{\bar{x},\ell} - R^{\mathcal F}_{m}\right)\\
	&\geq \maxErr{\mathcal{F},\bar{x}} - 2R^{\mathcal F}_{m} -2\left(\tilde{R}^{\mathcal F}_{\bar{x},\ell} - R^{\mathcal F}_{m}\right);\\
	&\geq \maxErr{\mathcal{F},\bar{x}} - 2\tilde{R}^{\mathcal F}_{\bar{x},\ell};
\end{align*} 
Further,
\begin{align*}
\sum_{i=1}^{m (\ell+1)}\Exp{Z_i^2} &= \sum_{i=1}^{m}\Exp{Z_i^2} + \sum_{i=m+1}^{m (\ell+1)} \Exp{Z_i^2};\\
& \leq m\frac{\ell + 4 +4\sqrt{\ell}}{4m^2\ell} + m\ell\frac{4}{m^2 \ell^2};\\
&\leq \frac{\ell + 4\sqrt{\ell}+20}{4m\ell}	
\end{align*} 
% $$\sum_{i=1}^{m (\ell+1)}\Exp{Z_i^2} = \sum_{i=1}^{m}\Exp{Z_i^2} + \sum_{i=m+1}^{m (\ell+1)} \Exp{Z_i^2}$$
% $$ \leq m\frac{\ell + 4 +4\ell}{4m^2\ell} + m\ell\frac{4}{m^2} 
% \leq \frac{\ell + 4\sqrt{\ell}+20}{4m\ell}.$$
% \end{align*} 
The statement follows.
\end{proof}

Due to its asymptotic nature, it is not possible to compare directly the tightness of the bound in Theorem~\ref{thm:mclrad} with that of finite sample bounds such as the one in Theorem~\ref{thm:bernmain}. Still, this bound is of great in many many practical scenarios as it allows for a much tighter bound for the generalization error.  

We note that the use of asymptotic bounds, is common practice in classical statistical tests (i.e., the \emph{student t\- test}, the \emph{z\- test}. Further, from our experimental results in Section~\ref{sec:exper}, we show how the bounds obtained using the MCLT are actually reliable in practice.

\subsection*{Comparison between approximations}
\begin{figure}[h!]\label{fig:comp}
\begin{center}
	\begin{tikzpicture}
  \begin{axis}[ 
    ylabel={$\Prob{R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}>\epsilon}$},
    xlabel={$\log_2 \ell$},
    xmin=1, xmax=6,
    ymin=0, %ymax=55,
    xtick={1,...,6},
    domain={1:6},
    samples=5,
    legend style={at={(1,0.4)},anchor=south east}
  ] 
    \addplot {e^(-2*1000*(e^x)*0.01^2/((e^x)+4))}; 
    \addplot {e^(-0.01^2/(5/(2*(e^x)*1000)))};
    \addplot {1-normcdf(0.01*2*((e^x)*1000/5)^0.5,0,1)};
    \addlegendentry{McDiarmid}
\addlegendentry{Bernstein}
\addlegendentry{MCLT}
  \end{axis}
\end{tikzpicture}
\end{center}
\caption{Comparison of the bound on the approximation of the \Rade of $\mathcal{F}$ using different techniques. Bounds are computed for a given sample of size $m = 1000$, for confidence level $\epsilon= 0.01$, and for various values of $\ell$.}
\end{figure}

In Figure~\ref{fig:comp} we present a comparison of the bounds on the quality of the estimation of the \Rade for $\mathcal{F}$ given by $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ obtained using applications of respectively McDiarmid's inequality (~\ref{lem:mcdiarmid2}), Bernstein's inequality (Lemma~\ref{lem:bernrade}), and the Martingale Central Limit Theorem (Lemma~\ref{lem:mcltrade}). 

While using a higher number $\ell$ of vectors of Rademacher random variables leads to an tighter bound for all approaches, the bound obtained with Bernstein's inequality and the MCLT decline much faster that the bound obtained using McDiarmid's inequality as $\ell$ increases. 

This is due to the fact that while the bounds obtained by applying Bernstein's inequality and the  \Rade approximation obtained using the MCLT depends on the second moment of the variation of the value of the function being considered (i.e., $\Exp{Z_i}$), the bound obtained McDiarmid's inequality depends  instead on the maximum variation of such value (i.e., $\max_{z\in\mathcal{X}, f\in \mathcal{F}} Z_i$).

Finally, the advantage of the bound achievable  using the MCLT rather than Bernstein's inequality is mainly due to the asymptotic nature of the MCLT bound rather than the finite sample nature of the bound which uses Bernstein's inequality.

==> 04_algo_old.tex <==
\section{The RADABOUND Algorithm}\label{sec:stopping}
The algorithm starts by drawing  $\ell$ \emph{independent} vectors of Rademacher variables. These vectors are fixed throughout the execution of the algorithm. The advantage of fixing the Rademacher vectors is that (1) we deal with a nested sequence of events, $\mathcal{F}_{k-1}\subseteq \mathcal{F}_{k}$, and (2) the actual computation of the Rademacher complexity estimate is simple and efficient. 

\paragraph{Computing the estimate:} 
%The actual computation of the estimate of the \Rade{} is very simple. 
At the end of each round $k$, the algorithm stores for each of the Rademacher vectors $j=1,\dots, \ell$, the value
%Given the dataset $\bar{x}$, for each of the $\ell$ instantiations of the vectors of Rademacher variables we store 
$\tilde{M}_{\bar{x},j}^{{\mathcal F}_{k}} =\max_{f\in \mathcal{ F}_k}
\frac{1}{|\bar{x}|}\sum_{i=1}^{|\bar{x}|} f(x_i)\mathbf{\sigma}_{i,j}$. 
To update these values, at iteration $k+1$, the algorithm computes 
$$\tilde{M}_{\bar{x},j}^{{\mathcal F}_{k+1}} \leftarrow \max \{\tilde{M}_{\bar{x},j}^{{\mathcal F}_{k}} , \frac{1}{|\bar{x}|}\sum_{i=1}^m f_{k+1}(x_i)\mathbf{\sigma}_{i,j}\}, ~~ j=1,\dots, \ell.$$
The estimate of the \Rade{} at round $k+1$ is then given by $\tilde{R}_{\bar{x}}^{{\mathcal F}_{k+1}}= \frac{1}{\ell} \sum_{j=1}^\ell \tilde{M}_{\bar{x},j}^{{\mathcal F}_{k+1}}$.

%%for $1\leq j \leq \ell$.
%At each step, when a new, adaptively chosen query $f_{k+1}$ is received, we can easily update each of these values:
%$$\tilde{M}_{\bar{x},j}^{{\mathcal F}_{k+1}} \leftarrow \max \{\tilde{M}_{\bar{x},j}^{{\mathcal F}_{k}} , \frac{1}{|\bar{x}|}\sum_{i=1}^m f_{k+1}(x_i)\mathbf{\sigma}_{i,j}\},$$
%The estimate of $R_{m}^{{\mathcal F}_{k+1}}$  is then computed as: $\tilde{R}_{\bar{x}}^{{\mathcal F}_{k+1}}= \frac{1}{\ell} \sum_{j=1}^\ell \tilde{M}_{\bar{x},j}^{{\mathcal F}_{k+1}}$.

\begin{algorithm}[ht]
\caption{RADABOUND - Adaptive data analysis with Rademacher Complexity control}\label{alg:RADABOUND}
\begin{algorithmic}[1]
\Procedure{RADABOUND}{$\bar{x},\varepsilon,\delta,\ell$}
%\State $\left(\Sam_p,\Samp_h\right) \leftarrow\ \textsc{RandSplit}(\Samp)$ 
\State $m\leftarrow \abs{\bar{x}}$ \Comment{Size of the input sample}
%\Comment{Initialization estimators for Rademacher Average}
\LeftComment{Initialization estimator for Rademacher Complexity}
\For{$j\in\{0,1,\ldots,\ell\}$} 
\State $\sigma_j \leftarrow $ vector of $m$ iid Rademacher RVs
\State $R^{\mathcal{F}_0}_{\bar{x},j}\leftarrow 0$
\EndFor 
%\State $\tilde{B}^{0}_{\bar{x}}\leftarrow 0$
%\State $\epsilon - \epsilon_{k,1}- 2\epsilon_{k,2}$
%\State $k\leftarrow 0$ 
%\Statex$\ $\Comment{Main execution body \hfill~}
\LeftComment{Main execution body}
\While{\text{new }k\text{-th  query} $f_k$ from the stream} 
	\State $\mathcal{F}_{k+1} \leftarrow \mathcal{F}_{k}\cup \{f_k\}$
	\LeftComment{Rademacher Average estimation update}
	\For{$j\in\{0,1,\ldots,\ell\}$} 
    %\Comment{Rademacher Complexity estimation update}
		\State $R_{\bar{x},j}^{{\mathcal F}_{k+1}} \leftarrow \max \{R_{\bar{x},j}^{{\mathcal F}_{k}} , \frac{1}{m} \sum_{i=1}^m f_k(x_i)\sigma_{j,i} \}$
	\EndFor
	\State $\tilde{R}_{\bar{x},\ell}^{{\mathcal F}_{k+1}} \leftarrow \frac{1}{\ell}\sum_{j=1}^\ell R_{\bar{x},j}^{{\mathcal F}_{k+1}}$
    \LeftComment{Control with BIM}
	\State \begin{varwidth}[t]{\linewidth}
	$\delta'\leftarrow \min_{\epsilon' \in \left(0, \epsilon-2\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}/2\right)}  e^{-2(\epsilon - 2\tilde{R}_{\bar{x},\ell}^{{\mathcal F}_{k+1}}-2\epsilon')^2m} + e^{\frac{6m \ell \epsilon'^2}{15+ 8\ell \epsilon'}}$\end{varwidth} 
    \LeftComment{Control with MCLT- Alternative to 11:}
    \State \begin{varwidth}[t]{\linewidth}{\bf or} $\delta'\leftarrow 1-\Phi\left( \max\{0, \epsilon-2\tilde{R}_{\bar{x},\ell}^{{\mathcal F}_{k+1}}\}\sqrt{\frac{4\ell m}{\ell + 4\sqrt{\ell}+20}} \right)$  \end{varwidth}
    %\Comment{Control with MCLT}% - Alternative to 11:}
%	\State $B^{k+1}_{\bar{x}}= \max \{B^{k}_{\bar{x}},      \left (\sum_{i=1}^m h^2(x_i)\right )^{\frac{1}{2}} \} $
%	\State $ \tilde{M}^{{\mathcal F}_{k+1}}_{\bar{x}} = \min[\tilde{R}^{{\mathcal F}_{k+1}}_{\bar{x}}, \frac{F^{k+1}_{\bar{x}}\sqrt{2\ln (k+1)}}{m}]$ %\Comment{Updating the Rademacher Complexity}
   % \State $\mathbf{amax} \leftarrow \textsc{UpdateMaxDiff}(\mathbf{\bar{a}},\mathbf{a}_k) $
   \LeftComment{Overfit control test}
    \If{$\delta' \leq \delta(1-\delta)$} %\hfill~}
    	\State{\textbf{return} $\frac{1}{m} \sum_{x \in \bar{x}} f(x)$}
    \Else
    	\State \begin{varwidth}[t]{\linewidth}\textbf{Halt: Cannot guarantee the statistical\\ validity of further queries.}\end{varwidth}
    \EndIf
\EndWhile
\EndProcedure
%\Statex
%\Procedure{EvaluateQuery}{$h,\Samp_h$}\Comment{Evaluate the ratio of correctly classified elements}
%\State \textbf{return} $\frac{1}{\abs{\Samp_h}}\sum\limits_{x\in \Samp_h} h\left(x\right)$
%\EndProcedure
%\Statex
\end{algorithmic}
\end{algorithm}
%Given the fact that in our setting we are using a sample $\bar{x}$ from ${\cal D}_k$ (rather than $\mathcal{D}$) to compute an approximation $R^{{\cal F}_{k+1}}_m$, we therefore have:
%\begin{align}\label{eqn:es2}
%&\Prob{\Psi ({\cal F}_k,\bar{x})\geq  \tilde{R}^{{\cal F}_{k+1}}_{\bar{x},\ell} + \epsilon_1+2\epsilon~|~E_k}\nonumber\\
%&\qquad \qquad \qquad \leq  \frac{e^{-2m\epsilon_1^2}+e^{-2m\ell\epsilon_2^2/\left(\ell+4\right)}}{\Probd{\mathcal D}{E_k}}.
%\end{align}
\paragraph{Stopping rule:}
%We are now ready to state a stopping rule for the adaptive inference process. 
Given real values $\epsilon,\delta \in (0,1)$, the procedure halts at the first ${k}$-th step for which it cannot guarantee that $\Probd{\mathcal{L}}{\Psi (\mathcal{ F}_{k+1},\bar{x}) > \epsilon} \leq \delta$. 
Recall from~\eqref{eq:iterativeproc} that 
%As discussed in~\eqref{eq:iterativeproc} this condition can also be expressed as:
\begin{equation}\label{eq:condstop2}
	\Probd{\mathcal{L}}{\Psi (\mathcal{ F}_k,\bar{x})> \epsilon}
\leq \frac{\Prob{\Psi (\mathcal{ F}_k,\bar{x})> \epsilon}}{\Prob{\Psi (\mathcal{ F}_{k-1},\bar{x})\leq \epsilon}}.
\end{equation}
Since $\Pr(\Psi (\mathcal{ F}_k,\bar{x})> \epsilon)\geq \Pr(\Psi (\mathcal{ F}_{k-1},\bar{x})> \epsilon)$, it is sufficient to require $\Prob{\Psi (\mathcal{ F}_k,\bar{x})>\epsilon}< \delta (1-\delta)$ to have $\Probd{\mathcal{L}}{\Psi (\mathcal{ F}_k,\bar{x})> \epsilon}\leq \delta,$ and we can use the bounds obtained in Theorem~\ref{thm:bernradetot} or Theorem~\ref{thm:mclrad}. Thus, we prove

%
%As $\mathcal{F}_{k-1}\subseteq \mathcal{F}_{k}$, we have that $\Pr_{\cal F}(\Psi ({\cal F}_k,\bar{x})> \epsilon)\geq \Pr_{\cal F}(\Psi ({\cal F}_{k-1},\bar{x})> \epsilon)$. 
%%(and thus, $\Pr_{\cal F}(\Psi ({\cal F}_k,\bar{x})\leq \epsilon)\leq \Pr_{\cal F}(\Psi ({\cal F}_{k-1},\bar{x})\leq \epsilon))$. 
%Therefore, if $\Prob{\Psi ({\cal F}_k,\bar{x})>\epsilon}< \delta (1-\delta)$, then we also have $\Probd{\mathcal{F}}{\Psi ({\cal F}_k,\bar{x})> \epsilon}\leq \delta.$
%
%Clearly $\Prob{\Psi ({\cal F}_k,\bar{x})>\epsilon}= \Prob{\Psi ({\cal F}_k,\bar{x})-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}>\epsilon-2\tilde{R}_{\bar{x},\ell}^{\mathcal{F}_k}}$. From Theorem~\ref{thm:bernradetot} we have:
%\begin{equation}\label{eq:stoppincon}
%\Prob{\Psi ({\cal F},\bar{x})- 2\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}>  \epsilon-2\tilde{R}^{\cal F_k}_{\bar{x},\ell}} <e^{-2m\left(\epsilon-2\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}-2\epsilon'\right)^2}+e^{\frac{6m \ell \epsilon'^2}{15+ 8\ell \epsilon'}},	
%\end{equation}
%	for $\epsilon' \in \left(0, \epsilon-2\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}/2\right)$.
%	
%At each step $k$, after updating the estimate of the \Rade{} for $\mathcal{F}_{k}$, \algo{} verifies wether there exists $\epsilon' \in (0, \epsilon-2\tilde{R}^{\mathcal{F}_k}_{\bar{x},\ell}/2)$ such that the right hand side of~\eqref{eq:stoppincon} is lower or equal to  $\delta(1-\delta)$. If that is the case, then \algo{} determines it is indeed possible to return the value if the $k$-th adaptively chosen query while maintaining the $\epsilon,\delta$ guarantees fixed by the user. Otherwise, the algorithm halts, as it determines that the condition in~\eqref{eq:stoppincon} is violated. Gathering these considerations, we can formally state the guarantees achieved by \algo{}:

\begin{theorem}
Given a sample $\bar{x}\sim\mathcal{D}^m$, let $\mathcal{F}_k$ denote the set of functions adaptively selected during the first $k$ steps. If \algo{} has not halted at step $k$,  then 
$$
\Probd{\mathcal{L}}{\Psi (\mathcal{ F}_k,\bar{x})\leq \epsilon} >1- \delta.
$$	
\end{theorem}
The bound in Theorem~\ref{thm:mclrad} based on the MCLT can be used in \algo{} \emph{as an alternative} to the bound in Theorem~\ref{thm:bernradetot} (lines 11-12 in Algorithm 1). In Section 5, we present an experimental comparison of performance of \algo{} when using the two methods.

==> 05_experiments_old.tex <==
\section{Experimental results}\label{sec:exper}
\begin{figure*}[ht]
\makebox[\textwidth][c]{
 \begin{minipage}{0.35\textwidth}
    %  \centering
\captionsetup{width=.85\linewidth}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/Bernn0_152.pdf}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/MCLTn0_2n}
\caption{MCLT}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{No signal. Feature values from $\mathcal{N}(0,1)$. $\delta = 0.1$.}
   \end{minipage}\hfill
\begin{minipage}{0.35\textwidth}
\captionsetup{width=.85\linewidth}
     \centering
     \begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/BER_0_15_tot1.pdf}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/MCLT_0_15_tot1}
\caption{MCLT bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{No signal. Feature values from $\mathcal{N}(0,2)$. $\delta = 0.15$.}
   \end{minipage}\hfill
\begin{minipage}{0.35\textwidth}
\captionsetup{width=.85\linewidth}
     \centering
     \begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/BERND20v8}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img/MCLTD20V8}
\caption{MCLT bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{No signal. Feature values from $\mathcal{N}(0,8)$. $\delta = 0.2$.}
   \end{minipage}
   }
\end{figure*}
We demonstrate the power and efficiency of our technique through a variety of experiments. Our experimental setup is similar to the one used in~\cite{Dwork15generalization}, except that all our reported results are for ranges of parameters for which we actually have provable statistical guarantees.

We consider a learning task of classifying vectors composed by $d$ features to the classes ``-1'' or ``1''.
%We consider a learning task of binary classifying of vectors of $d$ features.
We consider only linear classifier vectors $\textbf{w}\in \{-1,0,1\}^d$,  assigning vector $\textbf{x}$ to class $\textbf{h}(\textbf{x})= \textnormal{sign}\left(\textbf{w}\cdot\textbf{x}\right)$.
The goal of the learning algorithm is to find a classifier with minimum expected loss for the $0,1$ \emph{hard loss function} (0 for correct classification, 1 otherwise). To model a typical learning scenario, the learning algorithm is given two independent datasets.
A \emph{training set} $X_T$ and an \emph{holdout set} $X_H$. We then evaluate the performance of the learning  algorithm using a third, independent \emph{fresh set}.
% =============
% The goal of the algorithm being tested if to obtain a classifier $h()$ which ``\emph{fits the data}'' as best as possible, that is the a classifier which minimizes the \emph{Empirical Risk} over the holdout data, that is $\frac{1}{m} \sum_{\textbf{x}\in X_H} \ell\left(h(\textbf{x}), y(\textbf{x})\right)$, where $y(\textbf{x})$ denotes the ``\emph{true label}'' associated with the data point $\textbf{x}$ and $\ell\left(h(\textbf{x}), y(\textbf{x})\right)$ denotes the loss function. In our setting we consider the $\{0,1\}$ loss function such that $\ell\left(h(\textbf{x}), y(\textbf{x})\right)= 0$ if $h(\textbf{x}), y(\textbf{x}$ (i.e., the classifier $h()$ assigns the correct label to \textbf{x}), or  $\ell\left(h(\textbf{x}), y(\textbf{x})\right)= 1$ otherwise.

% The classifiers considered by the algorithm assign to each feature weights $w_i\in\{-1,0,1\}$. That is if a feature is selected with weight -1 (resp., 1) this indicates than the classifier assumes that the value of feature $w_i$ is negatively (rep., positively) correlated with the value of the label. If the classifier assigns weights 0, this corresponds to assuming that the value of a certain feature is not significant with respect to the value of the label. Given a classifier $\textbf{w}=\{-1,0,1\}^d$ and a point $\textbf{x}$, the label assigned by the algorithm is going to be $\textbf{w}(\textbf{x})= \textnormal{sign}\left(\textbf{w}\cdot\textbf{x}\right)$.

Our learning algorithm works as follows:
In the first phase, the algorithm  evaluates the correlation between the values of the features and the labels of the vectors using \emph{only} the training dataset $X_T$ as $c_i = \frac{1}{m} \sum_{\textbf{x}\in X_T} \textbf{x}[i]l(\textbf{x})$. The features are then sorted (in descending order) according to the absolute values of their correlations $|c_i|$ to the labels. %The highest correlation value first. 

The actual adaptive analysis of the data occurs in the second phase of the algorithm using the holdout data $X_H$. 
The algorithm starts with a classifier $\textbf{w}=0$. 
%with all weights $w_i$ set to zero. 
It then considers features according to the order computed in the  first phase. 
%That is, features with \emph{stronger} correlation (either positive or negative) to the label are considered first. 
Using the holdout set $X_H$,
the algorithm tests, for each feature, whether assigning weight -1 or 1 to it improves the performance of the current best classifier.
%among those evaluated so far in terms of empirical average error on the holdout dataset $X_H$.
If that is the case, the classifier is updated with the new value for the feature;
%is set to be new current risk minimizer, 
otherwise, the feature is left with weight zero. Each newly tested classifier is added to the class function $\mathcal{F}_k$. \algo{} then computes a new estimate $\tilde{R}_m^{\mathcal{F}_{k}}$ of the \Rade{} of $\mathcal{F}_k$, and uses it to determinate whether the total accumulated error is below $\epsilon$ with probability at least $1-\delta$ as discussed in Section~\ref{sec:stopping}.

%Our experiments consider two scenarios. In the first scenario, no feature is correlated with the vectors' labels. This scenario is best for measuring overfit to the holdout data. In the second scenario, some subset of features (unknown to the algorithm) is correlated (positively or negatively) with the labels. Experiments in this scenario demonstrate that controlling overfitting is not done at the expense of actually detecting the  signal in the data. 
Each figure above corresponds to several runs of an experiment with the same parameters but different values of $\epsilon$ (the error bound). The blue line gives the accuracy of the best classifier computed after running the corresponding number of queries on the holdout set $X_H$. The red line gives the accuracy of the same classifier on fresh data. The vertical bars give the computed stopping time for each value of $\epsilon$. The shaded green area corresponds to $\pm \epsilon$ values around the ``\emph{true accuracy}'' of the classifier (the red line), for the $\epsilon$ value of the next vertical bar. The green shaded area beyond the last bar uses the same $\epsilon$ as the last bar. 
In a correct execution of \algo{}, the blue line does not exit the green shaded area before the last vertical bar.
The power of \algo{} is measured by how close is the last bar to the first time the green line exit the shaded area. 

%In the experiments, we compare the results of \algo{}  when the error probability is estimated using (a) Bernstein's Inequality (Section~\ref{sec:bound}) and, (b) the Martingale Central Limit Theorem (Section~\ref{sec:mclt}).

In all the experiments $|X_T|=|X_H|= 4000$. Each vector in the dataset has 500 features. The estimation of the \Rade{} $\tilde{R}_{\bar{x},\ell}^{{\mathcal F}}$ is computed according to~\eqref{eq:radestimate} using $\ell =32$ vectors of Rademacher random variables. We report results using (a) Bernstein's Inequality (Section~\ref{sec:bound}) and, (b) the MCLT (Section~\ref{sec:mclt}).
%
%We verify the effectiveness of the Rademacher control using various parameters for $\delta$ and $\epsilon$. 
We consider the two following scenarios: 
%\vspace{-2.5mm}
%\begin{itemize}
%\item 

{\textbf{No signal in the data:}}
In this setting, each point $\textbf{x}\in X_H$ is assigned a label %``-1'' or ``1'' 
independently and uniformly at random. The feature values are taken \emph{independently} from a normal distribution with expectation 0 and various variance values. Thus, there is no correlation between the labels and the values of the features. We report the results in Figures 1-3.

% \begin{figure}[t]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/im_3.pdf}
%   \caption{Martingale Central Limit Theorem bound}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/im_4.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 1: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,4)$. $\delta = 0.1.$}
% \label{fig:fig2}
% \end{figure}
% \begin{figure}[H]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/im_1.pdf}
%   \caption{Martingale Central Limit Theorem bound}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/im_1b.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 2: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,8)$. $\delta = 0.1.$}
% \label{fig:fig2}
% \end{figure}

% \begin{figure}[t]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/img_5.pdf}
%   \caption{Martingale Central Limit Theorem estimation}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/img_6.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 3: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,16)$. $\delta = 0.3.$}
% \label{fig:fig2}
% \end{figure}

% The goal of the experiments is to show that as long as 
% \algo{} ensures that the constraint based on the Rademacher Complexity is maintained, no overfit
% higher than $\epsilon\in (0,1]$ is observed with probability at least $1-\delta$. 
% We report the results in Figures 1,2 and 4. In all the experiments $|X_T|=|X_H|= 4000$. Each vector in the dataset has 500 features which are each independent and identically distributed normal random variables with mean zero and various variances. We verify the effectiveness of the Rademacher control using various parameters for $\delta$ and $\epsilon$. 

% The green line represents the values of the current error minimizer. The red line represents the value of the function currently considered as the best (i.e., the current error minimizer) on a ``\emph{fresh}'' dataset $X_F$ drawn independently with respect the holdout set. Such dataset is used as a test for the generalization error of the current risk minimizer, in order to verify that our Rademacher Average test correctly halts once overfit is detected. For each experiment we present the results of the Rademacher control  when the the generalization error is bounded using (a) the approximation based on the application of the Martingale Central Limit Theorem (blue dashed lines), or (b) application of McDiarimid's inequality (magenta dashed lines). In particular, each vertical line marks the step $k$ at which the Rademacher control detects that a certain value of $\epsilon$ it is not possible to guarantee that $Pr(\Psi (\mathcal{ F}_k,\bar{x})\leq \epsilon)\geq 1 -\delta$. 
% When preceding a dashed line, the shaded green area denotes values within $\pm \epsilon'$ of the value of the current error minimizer when evaluated $X_F$, where $\epsilon'$ is the smallest value of $\epsilon$ among those considered for which it is still possible to guarantee that $Pr(\Psi ({\cal F}_k,\bar{x})\leq \epsilon')\geq 1 -\delta$. When placed after the last dashed line, the green area covers the $\pm \epsilon''$ of the value of the current error minimizer when evaluated $X_F$ where $\epsilon''$ is the last value for which the Rademacher control was active.
 
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.72\columnwidth]{img/noise8.pdf}
%   \caption{Exp. 3:  No signal in the data.  Values of the features from $\mathcal{N}(0,4)$, $\delta = 0.3$ using Martingale Central Limit Theorem estimation}
%   \label{fig:noisefig4}
% \end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.87\columnwidth]{img/noise7.pdf}
%   \caption{Exp. 5:  No signal in the data. $m=3000$, $d= 2000,$. Values of the features from $\mathcal{N}(0,16)$, $\delta = 0.1$ using Martingale Central Limit Theorem estimation}
%   \label{fig:noisefig4}
% \end{figure}
%\item 
{\textbf{Signal in the data:}}
\begin{figure*}[ht]
\makebox[\textwidth][c]{
   \begin{minipage}{0.335\textwidth}
   \captionsetup{width=.85\linewidth}
     \centering
     \begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/BernN04D01}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/MCLTN04D01}
\caption{MCLT bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{Signal. Feature values from $\mathcal{N}(0,4)$, $\delta = 0.1$, $bias = 0.5$.}
   \end{minipage}\hfill
 \begin {minipage}{0.335\textwidth}
 \captionsetup{width=.85\linewidth}
     \centering
     \begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/BernN05VD15B15}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/MCLTN05VD15B15}
\caption{MCLT bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{Signal. Feature values from $\mathcal{N}(0,2)$, $\delta = 0.15$, $bias = 0.5$.}
   \end{minipage}\hfill
   \begin {minipage}{0.335\textwidth}
   \captionsetup{width=.85\linewidth}
     \centering
     \begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/BernN08b500D2}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{img2/MCLTN08B500D2}
\caption{MCLT bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{Signal. Feature values from $\mathcal{N}(0,2)$, $\delta = 0.2$, $bias = 0.25$.}
   \end{minipage}
   }
\end{figure*}
%
%\begin{figure*}
%\centering
%\begin{minipage}{.3\textwidth}
%\centering
%\includegraphics[width=\textwidth]{img/noise8.pdf}
%  \caption{No signal in the data.  Values of the features from $\mathcal{N}(0,4)$, $\delta = 0.3$ using Martingale Central Limit Theorem bound.}
%  \label{fig:noisefig4}
%\end{minipage}\hfill
%\begin{minipage}{.3\textwidth}
%\centering
%\includegraphics[width=\textwidth]{img/imgs3}
%  \label{fig:sfig21}
%\caption{Signal in the data. Features from $\mathcal{N}(0,8)$. $20$ biased features, with bias$= 0.65$. $\delta = 0.2$ using Martingale Central Limit Theorem bound.}
%\label{fig:exp5}
%\end{minipage}\hfill
%\begin{minipage}{.3\textwidth}
%\centering
%\includegraphics[width=\textwidth]{img/imgs10.pdf}
%  \caption{Signal in the data.  Features from $\mathcal{N}(0,4)$. $12$ biased features, with bias$= 0.32$. $\delta = 0.2$ using Martingale Central Limit Theorem bound.}
%  \label{fig:exp6}
%\end{minipage}
%\end{figure*}
In this setting 
%there is actual correlation between the values of some of the features and the labels. The `
the ``\emph{strength}'' of the correlation between some features and the labels is characterized by two parameters: $n$, the number of the queries whose value is correlated to the label, and (positive or negative) $bias$ which defines the strength and sign of the correlation. We first generate datasets with no signal, like in the previous setting. We then fix a set of $50$  features to be  correlated with the label of their vectors. Letting $l(\textbf{x})$ be the label of vector $\textbf{x}$, the $50$ correlated features of $\textbf{x}$ are modified by adding $bias\times l(\textbf{x})$ to their original value. We report the results in Figures 4-6.
%\end{itemize}

% The goal of the experiments is to verify that, for given parameters $\epsilon,\delta \in (0,1)$, as long as 
% \algo{} ensures that the constraint based on the Rademacher Complexity is maintained, no overfit
% higher than $\epsilon$ is observed with probability at least $1-\delta$.

The results demonstrate that \algo{} successfully halts the sequence of tests before overfitting for the various values of $\epsilon$, as the green line corresponding to the values of the function evaluated on the holdout does not exit the green shaded area before the corresponding vertical bar. The statistical power of the procedure is highlighted in particular by the result of experiments for which there is actual correlation between the labels and the value of the features as the overfit control ensured by \algo{} is not achieved at the expense of detecting the  signal in the data.

In several scenarios, \algo{} halts its execution very close to the first iteration for which overfit (with respect to the value of $\epsilon$) actually occurs. \algo{} does not appear to be influenced by the distribution $\mathcal{D}$ over the data, but rather it behaves differently depending on the actual family of functions being tested. 

For similar $\epsilon, \delta$ parameters, the state-of-the-art $\mathtt{Thresholdout}$ algorithm~\cite{Dwork15generalization} would require an holdout dataset of size $\sim 4\times 10^6$ to provide answers to just 10 queries (details in Section~\ref{sec:dwork}). 
In contrast, our experiments show that \algo{} can provably handle such parameters with an holdout set of just 4000 samples, thus with an improvement of almost three orders of magnitude in terms of \emph{sample complexity}. The comparison is further discussed in Section~\ref{sec:dwork}.

Using the MCLT leads to a tight analysis of $\maxErr{\mathcal{ F}_k,\bar{x}}$, which in turn allows to test a higher number of adaptively chosen classifiers before halting and without overfitting (Figures 1-6b), compared to the stopping points obtained using the BIM (Figures 1-6a)\footnote{Using bounds obtained using McDiarmid's Inequality in \algo{} leads to stopping points considerably more conservative than those obtained using the BIM for the same parameters.}.

Finally, the fact that even when using the bounds obtained  using the MCLT, the procedure halts correctly, further suggests that, despite their ``asymptotic'' nature, these are actually highly reliable even when dealing with an input sample of relatively small dimension.  
%\subsection{Comparison with other methods}
%In this section we compare the performance of \algo{} with that of the standard Bonferroni
%correction (union bound) method, and the $\mathtt{Thresholdout}$ algorithm based on the concept of differential privacy.
%
%In Table 1 we compare the number of queries that each of the three methods can process with provable statistical guarantees for $m=3000$ and various 
%values of $\epsilon$ and $\delta$. The stopping times for \algo{} are taken from the experiments reported in Section~\ref{sec:exper} when using the bound based on the Martingale Central Limit. We explain below the computation of the values for the two other methods. 
%
%\begin{table}[h!]\label{table:qerinumbe}
%\centering
%\begin{tabular}{cccc}
%    \toprule
%     $\epsilon$ & \algo{} & $\mathtt{Thresholdout}$ & Bonferroni \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 1 (Figure 1) 1 $m=3000$, $\delta  =0.1$}\\ \midrule
%    $0.030$ & 5   & 0   & 4  \\
%    $0.035$ & 12   & 0   & 8  \\
%    $0.040$ & 22  & 0  & 9 \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 2 (Figure 2) 1 $m=3000$, $\delta  =0.1$}\\ \midrule 
%    $0.025$ & 5   & 0   & 4 \\
%    $0.030$ & 13   & 0   & 4  \\
%    $0.035$ & 112   & 0   & 8  \\
%    $0.040$ & 169  & 0  & 9 \\ \midrule
%%   \multicolumn{4}{l}{\ \ \ \ Experiment 3 (Figure 3) 1 $m=3000$, $\delta  =0.3$}\\ \midrule
%%     $0.025$ & 5   & 0   & 25 \\
%%     $0.030$ & 9   & 0   & 36  \\
%%     $0.035$ & 24   & 0   & 49  \\
%%     $0.040$ & 51  & 0  & 64 \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 5 (Figure 5) 1 $m=3000$, $\delta  =0.2$}\\ \midrule
%    $0.025$ & 5   & 0   & 9 \\
%    $0.030$ & 11   & 0   & 16  \\
%    $0.035$ & 40   & 0   & 20  \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 6 (Figure 6) 1 $m=3000$, $\delta  =0.2$}\\ \midrule
%    $0.025$ & 2   & 0   & 9 \\
%    $0.030$ & 5   & 0   & 16  \\
%    $0.035$ & 14   & 0   & 20  \\
%    $0.040$ & 313 & 0 & 25\\\bottomrule
%    \end{tabular}
%     \caption{Comparison of the number of statistically valid queries when using \algo{}, $\mathtt{Thresholdout}$ and Bonferroni.}
%\end{table}

%\subsection{Comparison with Differential Privacy based methods}
%\label{sec:dwork}
%% Dwork et al.~\cite{Dwork15generalization} presented the first applications of ``\emph{Differential Privacy}'' in the context of adaptive data analysis. In particular the 
%The $\mathtt{Thresholdout}$ algorithm~\cite{Dwork15generalization} provides guarantees similar to those of \algo{}. $\mathtt{Thresholdout}$ operates using two datasets: a public dataset and a private \emph{holdout} dataset. Every time a new query is received the algorithm evaluates its value on both the public and the private dataset. If their absolute difference is within a given \emph{threshold}, $\mathtt{Thresholdout}$ returns to the user the value observed on the public dataset after perturbing it with some noise. Viceversa, if the absolute difference is higher than a certain threshold, the algorithm detects that the query being considered is overfitting on the public dataset. In this case, $\mathtt{Thresholdout}$ may instead provide the value computed on the private dataset after perturbing it with noise. As this last operation effectively ``leaks'' information regarding the holdout it can be executed up to $B$ times, where $B$ must be fixed prior to the execution of the algorithm. 
%
%To characterize the number of queries for which algorithm $\mathtt{Thresholdout}$ provides provable statistical guarantees we apply Theorem 25 in~\cite{Dwork15generalization}~\footnote{A careful reader will notice that  Figures 1-3 in ~\cite{Dwork15generalization} (the same figure appears as Figures 1 and 2 in~\cite{dwork2015reusable}) represent an idealized illustration rather than statistically valid results. For the sample size used in these figures, the bound on the error probability of the threshold algorithm is not smaller than 1. Furthermore, the results crucially depend on a preprocessing of the two data sets (lines 95-97 in the ``runClassifier'' procedure in the python code in the supporting materials) that is not discussed in the paper.}. 
%%in evaluating  algorithm $\mathtt{Thresholdout}$ can process with the parameters in Table 1, and with $B=1$.
%The theorem states that 
%when testing up to $k$ queries, with up to $B=1$ of those being answered using the private ``Holdout set'',  the size of the holdout set must be at least:
%\begin{equation*}
%n \geq 96\epsilon^{-2}\ln\left(4k\delta^{-1}\right) \min\{80\sqrt{B\ln(1/\epsilon\delta) \}}, 16B\}
%\end{equation*}
%Thus, for $k = 10$, $B=1$, and $\epsilon = \delta = 0.1$: the required sample size is at least
%$$n\geq 100\times96\times \ln(400)\min\{80\sqrt{\ln(100)},16\} \geq 920288.$$ In contrast we showed in Section~\ref{sec:exper} that \algo{} can provably handle problems with these parameters with a sample size of just 3000. Further, $\mathtt{Thresholdout}$ requires that the user specifies before the execution the number of queries $k$ which are going to be adaptively chosen to be tested, and the number $B$ of maximum times that the algorithm can tolerate overfit on the public dataset by revealing information from the private ``\emph{holdout}'' dataset. 
%These requirements limit the adaptiveness of the process.
% In contrast \algo{} uses the holdout dataset \emph{as much as possible} without a fixed maximum number of queries. 
% Further, using \Rade{} allows to use the properties of the actual family of functions evaluated so far (i.e., their \emph{expressiveness}), rather than just its cardinality, in order to provide guarantees on the quality of the evaluations obtained in the adaptive analysis. 

%\subsection{Comparison with Bonferroni FWER control}
%We remark that classical FWER control techinques for the non-adaptive setting, such as the Bonferroni correction, cannot be applied to the adaptive setting. 

%\mynote[author=Lorenzo]{I think it would be important to clarify that it is indeed not possible to apply this method}
%Standard application of this method requires a $p$-values of each query. In our application the $p$-value is the probability that including an uncorrelated feature improves the performance of the algorithm on the holdout set. However, our requirement is less conservative. We can tolerate uncorrelated features in our classifier as long as the total error is bounded by $\epsilon$. 
%We therefore use in Table 1 a value $k$ such that the total bias  of $k$ uncorrelated features (with the appropriate weights) is greater than $\epsilon$ with probability at least $\delta$. We use Normal approximation to compute these values. We note that our bound is not tight. Some experiments show that this bound allows for too many queries. 


==> appcomp.tex <==
\section{Comparison between approximations}\label{app:comparison}
\begin{figure}
\begin{center}
	\begin{tikzpicture}
  \begin{axis}[ 
    ylabel={$\Prob{R^{\mathcal F}_{m}- \tilde{R}^{\mathcal F}_{\bar{x},\ell}>\epsilon}$},
    xlabel={$\log_2 \ell$},
    xmin=1, xmax=6,
    ymin=0, %ymax=55,
    xtick={1,...,6},
    domain={1:6},
    samples=5,
    legend style={at={(1,0.4)},anchor=south east}
  ] 
    \addplot {e^(-2*1000*(e^x)*0.01^2/((e^x)+4))}; 
    \addplot {e^(-0.01^2/(5/(2*(e^x)*1000)))};
    \addplot {1-normcdf(0.01*2*((e^x)*1000/5)^0.5,0,1)};
    \addlegendentry{McDiarmid}
\addlegendentry{Bernstein}
\addlegendentry{MCLT}
  \end{axis}
\end{tikzpicture}
\end{center}
\caption{Comparison of the bound on the approximation of the \Rade{} of $\mathcal{F}$ computed as $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ using different techniques. The bounds are computed for a given sample of size $m = 1000$, confidence level $\epsilon= 0.01$, and for various values of $\ell$.}\label{fig:comp}
\end{figure}

In Figure~\ref{fig:comp} we present a comparison of the bounds on the quality of the estimation of the \Rade for $\mathcal{F}$ given by $\tilde{R}^{\mathcal F}_{\bar{x},\ell}$ obtained using applications of respectively McDiarmid's inequality (Lemma~\ref{lem:mcdiarmid2}), Bernstein's inequality (Theorem~\ref{lem:bernrade}), and the Martingale Central Limit Theorem (Theorem~\ref{lem:mcltrade}). 

While using a higher number $\ell$ of vectors of Rademacher random variables leads to a tighter bound for all approaches, the bounds on the probability of overfitting obtained with Bernstein's inequality and the Martingale Central Limit Theorem decrease much faster than the bound obtained using McDiarmid's inequality as $\ell$ increases. 

This is due to the fact that while the bounds obtained by applying Bernstein's inequality and the  \Rade approximation obtained using the MCLT depends on the second moment of the variation of the value of the function being considered (i.e., $\Exp{Z_i}$), the bound obtained McDiarmid's inequality depends  instead on the maximum variation of such value (i.e., $\max_{z\in\mathcal{X}, f\in \mathcal{F}} Z_i$).

Finally, the advantage of the bound achievable  using the MCLT rather than Bernstein's inequality is mainly due to the asymptotic nature of the MCLT.
\clearpage

==> improved.tex <==
\section{Improved bounds for functions class with low Rademacher Complexity}

Using the same principle, if the function class $\mathcal{F}$ being considered exhibits lower variance, it is possible to achieve an overall tighter bound on the generalization error $\Psi ({\cal F},\bar{x})$.

\begin{theorem}\label{thm:improvbern}
\begin{equation*}
	\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}^{\cal F}_{\bar{x},\ell}+ \epsilon_3+2\epsilon_2}<e^{-2m\epsilon_2^2}+e^{-\frac{\epsilon^2}{\frac{5}{2\ell m }+\frac{4\epsilon_2}{3m}}}+e^{-\frac{\epsilon_3^2}{2mL+\frac{2\epsilon^3}{3m}}},
\end{equation*}
	where:
	\begin{align*}
		\tilde{L} &= \max_{f\in F} \frac{1}{m^2}\left( \frac{1}{m}\sum_{x_i\in \bar{x}} f'(x_i)+ 2\tilde{R}^{\cal F}_m+ \epsilon_1+2\epsilon_2 -\left(\frac{1}{m}\sum_{x_i\in \bar{x}} f'(x_i) - 2\tilde{R}^{\cal F}_m -\epsilon_1-2\epsilon_2\right)^2\right).
	\end{align*}
\end{theorem}
\begin{proof}
Let us consider the Doob martingale for the function $\maxErr{{\cal F},\bar{x}}$
\begin{equation}
C_i = \Exp{\maxErr{{\cal F},\bar{x}}|X_1,\ldots,X_i}
\end{equation}
which is defined with respect to the random variables $X_1,\ldots,X_m$ which correspond each to one of the elements in the sample $\bar{x}$. 
Let us consider the corresponding difference martingale $Z_i = C_{i+1}-C_{i}$. By linearity if expectation we have
\begin{equation*}
	Z_i = \frac{1}{m}\left(\Expe[f^*(x)] - f^*(X_i) \right),
\end{equation*}
where $f^*$ is the function among those in $\mathcal{F}$ which maximizes $\Expe{x\sim\mathcal{D}}{f(x)} - \frac{1}{|\bar{x}|}\sum_{x_i \in \bar{x} } f(x_i)$. As in our setting  the functions in $\mathcal{F}$ can only assume values $\{0,1\}$, we have that $Z_i\leq 1/m $ for all $i\in \{1,2,\ldots, m\}$.
In order to apply Bernstein's inequality for martingales we then need to bound the value of  $\sum_{i=1}^m\Exp{Z_i^2}$. We have:
\begin{align*}
\Exp{Z_i^2} &= \Exp{\left(\frac{\Exp{f^*(x)} - f^*(X_i)}{m^2}\right)^2}\\
	&= \frac{1}{m^2} \Exp{\Exp{f^*(x)}^2 + f^*(X_i)^2 -2\Exp{f^*(x)}  f^*(X_i)}
\end{align*}
By linearity of expectation we have:
\begin{align*}
\Exp{Z_i^2} &= \frac{1}{m^2}\left( \Exp{f^*(x)}^2 + \Exp{f^*(X_i)^2} -2\Exp{f^*(x)} \Exp{f^*(X_i)}\right)\\
&= \frac{1}{m^2}\left( \Exp{f^*(X_i)^2} -\Exp{f^*(x)}^2\right)
\end{align*}

As in our current setting we are considering functions which take values 0 or 1, we have $\Exp{f^*(X_i)^2} = \Exp{f^*(X_i)}$, and in turn:
\begin{equation}\label{eq:addres}
\Exp{Z_i^2} = \frac{1}{m^2}\left( \Exp{f^*(X_i)^2} -\Exp{f^*(x)}^2\right) = \frac{1}{m^2}\left( \Exp{f^*(X_i)} -\Exp{f^*(x)}^2\right).
\end{equation}
Let $f'$ denote the function in $\mathcal{F}$ which maximizes  $\Exp{f^*(X_i)} -\Exp{f^*(x)}^2$. Clearly:
\begin{equation*}
	\Exp{Z_i^2} \leq \frac{1}{m^2}\left( \Exp{f'(X_i)} -\Exp{f'(x)}^2\right)
\end{equation*}

According to the result of Theorem~\ref{thm:bernradetot}, we have that:
	\begin{equation*}
		\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}^{\cal F}_m+ \epsilon_1+2\epsilon_2}<e^{-2m\epsilon_1^2}+e^{\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}},
	\end{equation*}
and, hence:
\begin{equation*}
		\Prob{|\frac{1}{m}\sum_{i=1}^m f'(x_i)- \Expe{\cal D}{f'}| > 2\tilde{R}^{\cal F}_m+ \epsilon_1+2\epsilon_2}<e^{-2m\epsilon_1^2}+e^{\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}}. 
\end{equation*}
We can therefore use $\frac{1}{m}\sum_{x_i\in \bar{x}} f'(x_i)$ as an estimator for the value $\Expe{\cal D}{f'}$  in~\eqref{eq:addres}. Let:
\begin{equation*}
	L_i = \max_{f\in F} \frac{1}{m^2}\left( \frac{1}{m}\sum_{x_i\in \bar{x}} f'(x_i)+ 2\tilde{R}^{\cal F}_m+ \epsilon_1+2\epsilon_2 -\left(\frac{1}{m}\sum_{x_i\in \bar{x}} f'(x_i) - 2\tilde{R}^{\cal F}_m -\epsilon_1-2\epsilon_2\right)^2\right),
\end{equation*}
From Theorem~\ref{thm:bernradetot} we therefore have:
\begin{equation*}
	\Prob{\Exp{Z_i^2}> L} < e^{-2m\epsilon_1^2}+e^{\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}}.
\end{equation*}
and thus:
\begin{equation*}
	\Prob{\sum_{i=1}^m\Exp{Z_i^2}> mL} < e^{-2m\epsilon_1^2}+e^{\frac{6m \ell \epsilon_2^2}{15+ 8\ell \epsilon_2}}.
\end{equation*}
By applying Bernstein's inequality for martingales (i.e., ~\ref{thm:bern1bound}) we have:
\begin{equation*}
	\Prob{\Psi ({\cal F},\bar{x}) > \Exp{\Psi ({\cal F},\bar{x})}+ \epsilon_3}<e^{-\frac{\epsilon_3^2}{2\sum_{i=1}^m\Exp{Z_i^2}+\frac{2\epsilon^3 }{3m}}}
\end{equation*}
By combining this result with the result of Theorem~\ref{thm:bernmain} via the union bound we have:
\begin{equation*}
	\Prob{\Psi ({\cal F},\bar{x})> \Exp{\Psi ({\cal F},\bar{x})} +\epsilon_3} <e^{-2m\epsilon_2^2}+e^{-\frac{\epsilon^2}{\frac{5}{2\ell m }+\frac{4\epsilon_2}{3m}}}+e^{-\frac{\epsilon_3^2}{2mL+\frac{2\epsilon^3}{3m}}}
\end{equation*}
Further, from Theorem~\ref{thm:mainrade} we have:
\begin{equation*}
	\Prob{\Psi ({\cal F},\bar{x})> \Exp{\Psi ({\cal F},\bar{x})} +\epsilon_3} \leq \Prob{\Psi ({\cal F},\bar{x})> 2R^{\mathcal{F}}_{m} +\epsilon_3}.
\end{equation*}
Nohe that the in order for the result in Theorem~\ref{thm:bernradetot} to be verified, the result regarding the accuracy of the estimation of the Rademacher complexity in Theorem~\ref{lem:bernrade} has to be verifies as well. Hence we can conclude:
\begin{equation*}
	\Prob{\Psi ({\cal F},\bar{x}) > 2\tilde{R}^{\cal F}_{\bar{x},\ell}+ \epsilon_3+2\epsilon_2}<e^{-2m\epsilon_2^2}+e^{-\frac{\epsilon^2}{\frac{5}{2\ell m }+\frac{4\epsilon_2}{3m}}}+e^{-\frac{\epsilon_3^2}{2mL+\frac{2\epsilon^3}{3m}}}.
\end{equation*}
\end{proof}


==> macro.tex <==
% \usepackage[T1]{fontenc} % needed for lmodern
% \usepackage[utf8]{inputenc}
%\usepackage{lmodern} % More complete than the default CM font
% The following is to fix some font-shape missing warnings due to missing
% small-caps bold characters.
% \normalfont %to load T1lmr.fd
% \DeclareFontShape{T1}{lmr}{bx}{sc} { <-> ssub * cmr/bx/sc }{}
% \usepackage{dsfont} % for the indicator function
% \usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{subcaption}
%\usepackage[numbers,sort&compress,square]{natbib}
%\usepackage[hidelinks]{hyperref}
\usepackage{siunitx}
\usepackage{algorithm}
\floatname{algorithm}{ALGORITHM}
\usepackage[noend]{algpseudocode}
%\algrenewcommand\alglinenumber[1]{\small #1:}
%\usepackage{pifont}% http://ctan.org/pkg/pifont
%\usepackage{xspace}
\usepackage{float}

\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsthm}
%\newtheorem{fact}[theorem]{Fact}
\usepackage{mathrsfs}
\usepackage{pgfplots}
\usepackage{pgfmath}
\usepackage{varwidth}

\usepackage{float}
\newfloat{algorithm}{t}{lop}

\usepackage[show]{chato-notes}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}[section]

\newcommand{\Sam}{\mathcal{S}}
\newcommand{\DistP}{\mathcal{P}}
\newcommand{\Prob}[1]{\textrm{Pr}\left(#1\right)}
\newcommand{\Probd}[2]{\textrm{Pr}_{#1}\left(#2\right)}
\newcommand{\Exp}[1]{\text{E}\left[#1\right]}
\newcommand{\Expe}[2]{\text{E}_{#1}\left[#2\right]}
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}
\newcommand{\Expo}[1]{\exp\{#1\}}
\newcommand{\BO}[1]{O\left(#1\right)}

%\delimitershortfall-1sp
\newcommand\abs[1]{\left|#1\right|}

\newcommand{\seq}[3]{\mathbf{\text{#1}}_{#2}^{#3} }
\newcommand{\seque}[3]{\left(#1_{#2},\ldots,#1_{#3}\right) }

\newcommand{\gerr}[1]{R\left(#1\right)}
\newcommand{\terr}[2]{\widehat{R}_{#2}\left(#1\right)}
\newcommand{\loss}[2]{\ell\left(#1, #2\right)}

\newcommand{\Rade}{Rademacher Complexity}
\newcommand{\loga}[1]{\left(#1\right)}
\newcommand{\maxErr}[1]{\Psi\left(#1\right)}

\newcommand{\ExpApp}[1]{\tilde{\text{E}}\left[#1\right]}
\newcommand{\ExpeApp}[2]{\tilde{\text{E}}_{#1}\left[#2\right]}

%\def\cdf(#1)(#2)(#3){0.5*(1+(erf((#1-#2)/(#3*sqrt(2)))))}%
% to be used: \cdf(x)(mean)(variance)

%\DeclareMathOperator{\CDF}{cdf}
\tikzset{
    declare function={
        normcdf(\x,\m,\s)=1/(1 + exp(-0.07056*((\x-\m)/\s)^3 - 1.5976*(\x-\m)/\s));
    }
}
%\pgfplotsset{compat=1.13}
\makeatletter
\NewDocumentCommand{\LeftComment}{s m}{%
  \Statex \IfBooleanF{#1}{\hspace*{\ALG@thistlm}}\(\triangleright\) #2}
\makeatother 

==> oldexp.tex <==
\section{Experimental results}\label{sec:exper}
We demonstrate the power and efficiency of our technique through a variety of experiments. Our experimental setup is similar to the one used in~\cite{Dwork15generalization}, with the exception that we only report results in ranges of parameters for which we have provable statistical guarantees.

We consider a learning task of classifying vectors composed by $d$ features to the classes ``-1'' or ``1''. We consider only linear classifier vectors $\textbf{w}\in \{-1,0,1\}^d$,  assigning vector $\textbf{x}$ to class $\textbf{h}(\textbf{x})= \textnormal{sign}\left(\textbf{w}\cdot\textbf{x}\right)$.
The goal of the learning algorithm is to minimize the expected loss for the standard $0,1$ \emph{hard loss} function (0 for correct classification, 1 otherwise).

To model a typical learning scenario the learning algorithm is given two independent datasets.
A \emph{training set} $X_T$ and an \emph{holdout set} $X_H$. We then evaluate the performance of the learning  algorithm using a third, independent, \emph{fresh set}.
% =============
% The goal of the algorithm being tested if to obtain a classifier $h()$ which ``\emph{fits the data}'' as best as possible, that is the a classifier which minimizes the \emph{Empirical Risk} over the holdout data, that is $\frac{1}{m} \sum_{\textbf{x}\in X_H} \ell\left(h(\textbf{x}), y(\textbf{x})\right)$, where $y(\textbf{x})$ denotes the ``\emph{true label}'' associated with the data point $\textbf{x}$ and $\ell\left(h(\textbf{x}), y(\textbf{x})\right)$ denotes the loss function. In our setting we consider the $\{0,1\}$ loss function such that $\ell\left(h(\textbf{x}), y(\textbf{x})\right)= 0$ if $h(\textbf{x}), y(\textbf{x}$ (i.e., the classifier $h()$ assigns the correct label to \textbf{x}), or  $\ell\left(h(\textbf{x}), y(\textbf{x})\right)= 1$ otherwise.

% The classifiers considered by the algorithm assign to each feature weights $w_i\in\{-1,0,1\}$. That is if a feature is selected with weight -1 (resp., 1) this indicates than the classifier assumes that the value of feature $w_i$ is negatively (rep., positively) correlated with the value of the label. If the classifier assigns weights 0, this corresponds to assuming that the value of a certain feature is not significant with respect to the value of the label. Given a classifier $\textbf{w}=\{-1,0,1\}^d$ and a point $\textbf{x}$, the label assigned by the algorithm is going to be $\textbf{w}(\textbf{x})= \textnormal{sign}\left(\textbf{w}\cdot\textbf{x}\right)$.

Our learning algorithm works as follows:
In first phase the algorithm  evaluates the correlation between the values of the features and the labels of the vectors using \emph{only} the training dataset $X_T$ as $c_i = \frac{1}{m} \sum_{\textbf{x}\in X_T} \textbf{x}[i]l(\textbf{x})$. The features are then sorted according to the absolute values $|c_i|$. The highest value first. 

The second, main phase of the algorithm, is the one in which the actual adaptive analysis of the data occurs using the holdout data $X_H$. 
The algorithm starts with a classifier with all weights $w_i$ set to zero. It then considers features according to the order computed in the  first phase. That is, features with \emph{stronger} correlation (either positive or negative) to the label are considered first. For each feature, the algorithm tests, using the holdout set,
whether assigning weight -1 or 1 to it improves of the performance of the current best classifier among those evaluated so far in terms of empirical average error on the holdout dataset $X_H$. If that is the case, then the new classifier is set to be new current risk minimizer, otherwise, the feature is left with weight zero.

Each newly tested classifier is added to the class function $\mathcal{F}_k$. \algo{} then computes a new estimate $\tilde{R}_m^{\mathcal{F}_{k}}$ of and uses is to determinate wether the total accumulated error is below $\epsilon$ with probability at least $1-\delta$, according to the strategy discussed in Section~\ref{sec:stopping}.

%Our experiments consider two scenarios. In the first scenario, no feature is correlated with the vectors' labels. This scenario is best for measuring overfit to the holdout data. In the second scenario, some subset of features (unknown to the algorithm) is correlated (positively or negatively) with the labels. Experiments in this scenario demonstrate that controlling overfitting is not done at the expense of actually detecting the  signal in the data. 
Each figure in this section corresponds to several runs of an experiment with the same parameters but different values of $\epsilon$ (the error bound). The green line gives the accuracy of the best classifier computed after running the corresponding number of queries on the holdout set $X_H$. The red line gives the accuracy of the same classifier on fresh data. The vertical bars give the computed stopping time for each value of $\epsilon$. The shaded green area corresponds to $\pm \epsilon$ values around the true accuracy of the classifier (the red line), for the $\epsilon$ value of the next vertical bar. The green shaded area beyond the last bar uses the same $\epsilon$ as the last bar.

In a correct execution of \algo{}, the blue line does not exit the green shaded area before the last vertical bar.
 The power of \algo{} is measured by how close is the last bar to the first time the green line exit the shaded area. In the experiments we compare the results of \algo{}  when the error probability is estimated using (a) Bernstein's inequality for Martingales (Section~\ref{sec:bound}); and, (b) the Martingale Central Limit Theorem (Section~\ref{sec:mclt}).

\paragraph{No signal in the data:}
\begin{figure*}
\centering
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{img/BER_0_15_tot1.pdf}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{img/MCLT_0_15_tot1}
\caption{Central Limit Theorem bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{Features values sampled from $\mathcal{N}(0,2)$. $\delta = 0.15$.}
\end{figure*}
\begin{figure*}
\centering
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{img/Bernn0_152.pdf}
\caption{Bernstein bound}
\label{fig:exp1}
\end{subfigure}\hfill
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{img/MCLTn0_2n}
\caption{Central Limit Theorem bound}
\label{fig:exp2}
\end{subfigure}\hfill
\caption{Features values sampled from $\mathcal{N}(0,1)$. $\delta = 0.1$.}
\end{figure*}
In this setting each point $\textbf{x}\in X_H$ is assigned label ``-1'' or ``1'' independently and uniformly at random. The $d$ feature values are taken \emph{independently} from a Normal distribution with expectation 0 and various standard variation values. Thus, there is no correlation between the labels and any feature of the vectors. 


% \begin{figure}[t]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/im_3.pdf}
%   \caption{Martingale Central Limit Theorem bound}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/im_4.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 1: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,4)$. $\delta = 0.1.$}
% \label{fig:fig2}
% \end{figure}
% \begin{figure}[H]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/im_1.pdf}
%   \caption{Martingale Central Limit Theorem bound}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/im_1b.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 2: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,8)$. $\delta = 0.1.$}
% \label{fig:fig2}
% \end{figure}

% \begin{figure}[t]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/img_5.pdf}
%   \caption{Martingale Central Limit Theorem estimation}
%   \label{fig:sfig1}
% \end{subfigure}%
% \hfill
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=.75\linewidth]{img/img_6.pdf}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig2}
% \end{subfigure}
% \caption{Exp. 3: no signal in the data. $m=3000$, $d= 400,$. Value of the features from $\mathcal{N}(0,16)$. $\delta = 0.3.$}
% \label{fig:fig2}
% \end{figure}
The goal of the experiments is to show that as long as 
\algo{} ensures that the constraint based on the Rademacher Complexity is maintained, no overfit
higher than $\epsilon\in (0,1]$ is observed with probability at least $1-\delta$. 
We report the results in Figures 1,2 and 4. In all the experiments $|X_T|=|X_H|= 4000$. Each vector in the dataset has 500 features which are each independent and identically distributed normal random variables with mean zero and various variances. We verify the effectiveness of the Rademacher control using various parameters for $\delta$ and $\epsilon$. 
% The green line represents the values of the current error minimizer. The red line represents the value of the function currently considered as the best (i.e., the current error minimizer) on a ``\emph{fresh}'' dataset $X_F$ drawn independently with respect the holdout set. Such dataset is used as a test for the generalization error of the current risk minimizer, in order to verify that our Rademacher Average test correctly halts once overfit is detected. For each experiment we present the results of the Rademacher control  when the the generalization error is bounded using (a) the approximation based on the application of the Martingale Central Limit Theorem (blue dashed lines), or (b) application of McDiarimid's inequality (magenta dashed lines). In particular, each vertical line marks the step $k$ at which the Rademacher control detects that a certain value of $\epsilon$ it is not possible to guarantee that $Pr(\Psi ({\cal F}_k,\bar{x})\leq \epsilon)\geq 1 -\delta$. 
% When preceding a dashed line, the shaded green area denotes values within $\pm \epsilon'$ of the value of the current error minimizer when evaluated $X_F$, where $\epsilon'$ is the smallest value of $\epsilon$ among those considered for which it is still possible to guarantee that $Pr(\Psi ({\cal F}_k,\bar{x})\leq \epsilon')\geq 1 -\delta$. When placed after the last dashed line, the green area covers the $\pm \epsilon''$ of the value of the current error minimizer when evaluated $X_F$ where $\epsilon''$ is the last value for which the Rademacher control was active.

The results demonstrate that \algo{} successfully halts the sequence of tests before overfitting for the various values of $\epsilon$, as the green line corresponding to the values of the function evaluated on the holdout does not exit the green shaded area before the corresponding vertical bar. Furthermore  the estimates using the Martingale Central Limit theorem leads to a tight analysis which in turn allow to test a higher number of adaptively chosen classifiers before halting and without overfitting (Figures 1b, 2b), compared to the stopping points obtained using the bound given by Bernstein's inequality (Figures 1a, 2a)\footnote{Using bounds obtained using McDiarmid's inequality in \algo{} for the same parameters leads to stopping points considerably more conservatvive than those obtained using the Bernstein bound.}

In several scenarios \algo{} halts its execution very close to the first iteration for which overfit (with respect to the value of $\epsilon$) actually occurs. \algo{} does not appear to be influenced by the distribution $\mathcal{D}$ over the data, but rather it behaves differently depending on the actual family of functions being tested.  
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.72\columnwidth]{img/noise8.pdf}
%   \caption{Exp. 3:  No signal in the data.  Values of the features from $\mathcal{N}(0,4)$, $\delta = 0.3$ using Martingale Central Limit Theorem estimation}
%   \label{fig:noisefig4}
% \end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.87\columnwidth]{img/noise7.pdf}
%   \caption{Exp. 5:  No signal in the data. $m=3000$, $d= 2000,$. Values of the features from $\mathcal{N}(0,16)$, $\delta = 0.1$ using Martingale Central Limit Theorem estimation}
%   \label{fig:noisefig4}
% \end{figure}

\subsection{Signal in the data}
\begin{figure*}[ht]
\centering
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\textwidth]{img/noise8.pdf}
  \caption{No signal in the data.  Values of the features from $\mathcal{N}(0,4)$, $\delta = 0.3$ using Martingale Central Limit Theorem bound.}
  \label{fig:noisefig4}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\textwidth]{img/imgs3}
  \label{fig:sfig21}
\caption{Signal in the data. Features from $\mathcal{N}(0,8)$. $20$ biased features, with bias$= 0.65$. $\delta = 0.2$ using Martingale Central Limit Theorem bound.}
\label{fig:exp5}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=\textwidth]{img/imgs10.pdf}
  \caption{Signal in the data.  Features from $\mathcal{N}(0,4)$. $12$ biased features, with bias$= 0.32$. $\delta = 0.2$ using Martingale Central Limit Theorem bound.}
  \label{fig:exp6}
\end{minipage}
\end{figure*}
Next, we test the performance of our algorithm when there is an actual correlation between the values of some of the features and the labels. The ``\emph{strength}'' of such correlation is characterized by two parameters: $n$ the number of the queries whose value is correlated to the label, and (positive or negative) $bias$ which defines the strength and sign of the correlation. 

The datasets are generated as follows: We first generate datasets with no signal, similar to the ones used in the previous section. We then fix a set of $n$  features to be  correlated with the label of their vectors. Let $l(\textbf{x})$ be the label of vector $\textbf{x}$. The $n$ correlated features of $\textbf{x}$ are modified by adding $bias\times l(\textbf{x})$ to their original value. In all the experiments $|X_T|=|X_H|= 3000$. The vectors in the dataset have 500 features each. 
% \begin{figure}[h]
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/imgs100}
%   \caption{Martingale Central Limit Theorem bound.}
%   \label{fig:sfig21}
% \end{subfigure}%
% \hfill
% % \begin{subfigure}{.45\textwidth}
% %   \centering
% %   \includegraphics[width=.9\linewidth]{img/imgs1}
% %   \caption{Martingale Central Limit Theorem bound.}
% %   \label{fig:sfig22}
% % \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.75\textwidth]{img/img100mc}
%   \caption{Mc Diarmid's inequality bound}
%   \label{fig:sfig23}
% \end{subfigure}%
% % \begin{subfigure}{.5\textwidth}
% %   \centering
% %   \includegraphics[width=.9\linewidth]{img/img1mc}
% %   \caption{Mc Diarmid's inequality bound}
% %   \label{fig:sfig24}
% % \end{subfigure}
% \caption{Exp. 6: Signal in the data. $m=3000$, $d= 500,$. Value of the features from $\mathcal{N}(0,4)$. $25$ biased features, with bias$= 0.35$. $\delta = 0.2$}
% \label{fig:fig4}
% \end{figure}

% \begin{figure}[h]
% %\begin{subfigure}{0.45\textwidth}
%   \centering
%   \includegraphics[width=0.72\columnwidth]{img/imgs3}
%   \label{fig:sfig21}
% \caption{Exp. 5: Signal in the data. Features from $\mathcal{N}(0,8)$. $20$ biased features, with bias$= 0.65$. $\delta = 0.2$}
% \label{fig:exp5}
% \end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.72\columnwidth]{img/imgs10.pdf}
%   \caption{Exp. 6:  Signal in the data.  Features from $\mathcal{N}(0,4)$. $12$ biased features, with bias$= 0.32$. $\delta = 0.2$ using Martingale Central Limit Theorem estimation}
%   \label{fig:exp6}
% \end{figure}
% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.8\columnwidth]{img/imgs20.pdf}
%   \caption{Exp. 9:  Signal in the data. $m=3000$, $d= 500,$. Value of the features from $\mathcal{N}(0,4)$. $12$ biased features, with bias$= 0.32$. $\delta = 0.2$ using Martingale Central Limit Theorem estimation}
%   \label{fig:sfig1}
% \end{figure}

The results presented in Figures 3,5 and 6, verify that \algo{} successfully halts the testing procedure before overfit for various values of $\epsilon$. These results further demonstrate the statistical power of the procedure. Overfit control is not done at the expense of detecting the  signal in the data. Our results also shows that the asymptotic MCLT are indeed valid for small data of a few thousands points).

% This further suggests that while the bounds obtained using the MCLT are of asymptotic nature (as opposed to the finite sample bounds obtainable using McDiarmid's inequality), they are actually extremely rigorous even when dealing with an input sample of relatively small dimension (i.e., e few thousands points).  
%\subsection{Comparison with other methods}
%In this section we compare the performance of \algo{} with that of the standard Bonferroni
%correction (union bound) method, and the $\mathtt{Thresholdout}$ algorithm based on the concept of differential privacy.
%
%In Table 1 we compare the number of queries that each of the three methods can process with provable statistical guarantees for $m=3000$ and various 
%values of $\epsilon$ and $\delta$. The stopping times for \algo{} are taken from the experiments reported in Section~\ref{sec:exper} when using the bound based on the Martingale Central Limit. We explain below the computation of the values for the two other methods. 
%
%\begin{table}[h!]\label{table:qerinumbe}
%\centering
%\begin{tabular}{cccc}
%    \toprule
%     $\epsilon$ & \algo{} & $\mathtt{Thresholdout}$ & Bonferroni \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 1 (Figure 1) 1 $m=3000$, $\delta  =0.1$}\\ \midrule
%    $0.030$ & 5   & 0   & 4  \\
%    $0.035$ & 12   & 0   & 8  \\
%    $0.040$ & 22  & 0  & 9 \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 2 (Figure 2) 1 $m=3000$, $\delta  =0.1$}\\ \midrule 
%    $0.025$ & 5   & 0   & 4 \\
%    $0.030$ & 13   & 0   & 4  \\
%    $0.035$ & 112   & 0   & 8  \\
%    $0.040$ & 169  & 0  & 9 \\ \midrule
%%   \multicolumn{4}{l}{\ \ \ \ Experiment 3 (Figure 3) 1 $m=3000$, $\delta  =0.3$}\\ \midrule
%%     $0.025$ & 5   & 0   & 25 \\
%%     $0.030$ & 9   & 0   & 36  \\
%%     $0.035$ & 24   & 0   & 49  \\
%%     $0.040$ & 51  & 0  & 64 \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 5 (Figure 5) 1 $m=3000$, $\delta  =0.2$}\\ \midrule
%    $0.025$ & 5   & 0   & 9 \\
%    $0.030$ & 11   & 0   & 16  \\
%    $0.035$ & 40   & 0   & 20  \\ \midrule
%    \multicolumn{4}{l}{\ \ \ \ Experiment 6 (Figure 6) 1 $m=3000$, $\delta  =0.2$}\\ \midrule
%    $0.025$ & 2   & 0   & 9 \\
%    $0.030$ & 5   & 0   & 16  \\
%    $0.035$ & 14   & 0   & 20  \\
%    $0.040$ & 313 & 0 & 25\\\bottomrule
%    \end{tabular}
%     \caption{Comparison of the number of statistically valid queries when using \algo{}, $\mathtt{Thresholdout}$ and Bonferroni.}
%\end{table}

%\subsection{Comparison with Differential Privacy based methods}
%\label{sec:dwork}
%% Dwork et al.~\cite{Dwork15generalization} presented the first applications of ``\emph{Differential Privacy}'' in the context of adaptive data analysis. In particular the 
%The $\mathtt{Thresholdout}$ algorithm~\cite{Dwork15generalization} provides guarantees similar to those of \algo{}. $\mathtt{Thresholdout}$ operates using two datasets: a public dataset and a private \emph{holdout} dataset. Every time a new query is received the algorithm evaluates its value on both the public and the private dataset. If their absolute difference is within a given \emph{threshold}, $\mathtt{Thresholdout}$ returns to the user the value observed on the public dataset after perturbing it with some noise. Viceversa, if the absolute difference is higher than a certain threshold, the algorithm detects that the query being considered is overfitting on the public dataset. In this case, $\mathtt{Thresholdout}$ may instead provide the value computed on the private dataset after perturbing it with noise. As this last operation effectively ``leaks'' information regarding the holdout it can be executed up to $B$ times, where $B$ must be fixed prior to the execution of the algorithm. 
%
%To characterize the number of queries for which algorithm $\mathtt{Thresholdout}$ provides provable statistical guarantees we apply Theorem 25 in~\cite{Dwork15generalization}~\footnote{A careful reader will notice that  Figures 1-3 in ~\cite{Dwork15generalization} (the same figure appears as Figures 1 and 2 in~\cite{dwork2015reusable}) represent an idealized illustration rather than statistically valid results. For the sample size used in these figures, the bound on the error probability of the threshold algorithm is not smaller than 1. Furthermore, the results crucially depend on a preprocessing of the two data sets (lines 95-97 in the ``runClassifier'' procedure in the python code in the supporting materials) that is not discussed in the paper.}. 
%%in evaluating  algorithm $\mathtt{Thresholdout}$ can process with the parameters in Table 1, and with $B=1$.
%The theorem states that 
%when testing up to $k$ queries, with up to $B=1$ of those being answered using the private ``Holdout set'',  the size of the holdout set must be at least:
%\begin{equation*}
%n \geq 96\epsilon^{-2}\ln\left(4k\delta^{-1}\right) \min\{80\sqrt{B\ln(1/\epsilon\delta) \}}, 16B\}
%\end{equation*}
%Thus, for $k = 10$, $B=1$, and $\epsilon = \delta = 0.1$: the required sample size is at least
%$$n\geq 100\times96\times \ln(400)\min\{80\sqrt{\ln(100)},16\} \geq 920288.$$ In contrast we showed in Section~\ref{sec:exper} that \algo{} can provably handle problems with these parameters with a sample size of just 3000. Further, $\mathtt{Thresholdout}$ requires that the user specifies before the execution the number of queries $k$ which are going to be adaptively chosen to be tested, and the number $B$ of maximum times that the algorithm can tolerate overfit on the public dataset by revealing information from the private ``\emph{holdout}'' dataset. 
%These requirements limit the adaptiveness of the process.
% In contrast \algo{} uses the holdout dataset \emph{as much as possible} without a fixed maximum number of queries. 
% Further, using \Rade{} allows to use the properties of the actual family of functions evaluated so far (i.e., their \emph{expressiveness}), rather than just its cardinality, in order to provide guarantees on the quality of the evaluations obtained in the adaptive analysis. 

%\subsection{Comparison with Bonferroni FWER control}
%We remark that classical FWER control techinques for the non-adaptive setting, such as the Bonferroni correction, cannot be applied to the adaptive setting. 

%\mynote[author=Lorenzo]{I think it would be important to clarify that it is indeed not possible to apply this method}
%Standard application of this method requires a $p$-values of each query. In our application the $p$-value is the probability that including an uncorrelated feature improves the performance of the algorithm on the holdout set. However, our requirement is less conservative. We can tolerate uncorrelated features in our classifier as long as the total error is bounded by $\epsilon$. 
%We therefore use in Table 1 a value $k$ such that the total bias  of $k$ uncorrelated features (with the appropriate weights) is greater than $\epsilon$ with probability at least $\delta$. We use Normal approximation to compute these values. We note that our bound is not tight. Some experiments show that this bound allows for too many queries. 
